Data Leakage in Notebooks: Static Detection and Better Processes

Data science pipelines to train and evaluate models with machine learning may contain bugs just like any other code. Leakage between training and test data can lead to overestimating the model's accuracy during offline evaluations, possibly leading to deployment of low-quality models in production. Such leakage can happen easily by mistake or by following poor practices, but may be tedious and challenging to detect manually. We develop a static analysis approach to detect common forms of data leakage in data science code. Our evaluation shows that our analysis accurately detects data leakage and that such leakage is pervasive among over 100,000 analyzed public notebooks. We discuss how our static analysis approach can help both practitioners and educators, and how leakage prevention can be designed into the development process.

==> body/1-introduction.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}
\begin{lstlisting}[language=Python] 
import numpy as np
# generate random data
n_samples, n_features, n_classes = 200, 10000, 2
rng = np.random.RandomState(42)
X = rng.standard_normal((n_samples, n_features))
y = rng.choice(n_classes, n_samples)

# leak test data through feature selection
X_selected = SelectKBest(k=25).fit_transform(X, y)

X_train, X_test, y_train, y_test = train_test_split(
    X_selected, y, random_state=42)
gbc = GradientBoostingClassifier(random_state=1)
gbc.fit(X_train, y_train)

y_pred = gbc.predict(X_test)
accuracy_score(y_test, y_pred)  
# expected accuracy ~0.5; reported accuracy 0.76
\end{lstlisting}
\vspace{-1em}
\caption{Data leakage may cause a highly-biased test result.
The model learns test data distribution through feature selection,
resulting in an over-optimistic test score.
}
\label{fig:leak_acc}
\vspace{-1.5em}
\end{figure}


Will a promising machine-learned model work when deployed in production? 
Typically this question is answered by comparing model predictions to expected outcomes on test data.
However, the resulting accuracy estimates can be misleading, where the model performs well on test data, but much worse in production. 
A common cause is that the data used for testing is not representative enough of the production data, thus providing misleading estimates on the wrong data distribution. 
A different cause, and the focus of this paper, is that the test data was used in some form during model training (directly or indirectly, intentionally or accidentally) allowing the model to overfit on the test data, thus producing unrealistically optimistic accuracy estimates. Because data science pipelines are code, we can use software engineering techniques to analyze them---which we do in this paper.

In this paper, we design a static analysis approach to detect cases where model training makes use of test data in data science code, commonly called \emph{data leakage}~\cite{kaufman2012leakage, burkov2020machine}. Data leakage is often the result of using bad practices when writing machine learning code, ranging from obvious mistakes, such as including test data in the training data, to more subtle ones that leak test data distribution information through preprocessing prior to training. For example, in Fig.~\ref{fig:leak_acc}, we show data science code reporting confidently to find patterns in random data where the model should not do better than a random guess: Because decisions during training depend on both training and test data (feature selection, Line~9) the model overfits on test data and the evaluation reports significantly inflated accuracy scores. Our analysis points out common pitfalls in model accuracy evaluations like the one in our example, which, as we will show, are pervasive in data science code in public notebooks.

Our analysis has both practical and educational value. On the practical side, our work contributes to more reliable offline evaluations of machine-learned models, which are an important quality assurance step when integrating models into software products. Use of machine learning in software products is increasingly common, but also very challenging~\cite{nadiaICSE22,microsoftSE4MLpaper,hulten2018building}. Reliable offline accuracy evaluations are important for preventing harm from deploying low-quality models in production systems, where harm can range from stress, to discrimination, to fatal accidents~\cite{amazon-bias, tesla-crash}.
Accuracy results are also a common quality metric between teams~\cite{nadiaICSE22}, especially when delegating or entirely outsourcing model development. When accuracy goals are parts of contracts (or competitions) there may be an incentive to report inflated accuracy results.

\looseness=-1
On the educational side, the danger of overfitting and data leakage is well known and commonly discussed in textbooks~\cite{MLtextbook, burkov2020machine}, ML library documentation~\cite{scikit, imblearn}, and tutorials~\cite{alexisbcook_2021}. Yet, as we will show, leakage also occurs in tutorial notebooks, popular notebooks, and entries in data science competitions, which others may use as educational resources or templates. Our analysis, just like other static analyses, can help raise awareness of coding problems and nudge students and model developers toward better practices.

Technically, we develop a static data-flow analysis that tracks how datasets flow through data science code and are used in training and evaluation functions of machine-learning libraries. To allow accurate detection, we track specific kinds of transformations and detect common patterns that lead to leakage. In an evaluation with data science code from public notebooks, we show that our analysis is accurate (92.9\%) with very few false positives and can analyze most notebooks within a few seconds. Applying our analysis to over 100,000 public notebooks, we detect data leakage issues in nearly 30~percent of them.

In summary, we make the following contributions:
\begin{itemize}
    \item  A summary and formulation of common data leakage problems.
\item A static analysis that can automatically detect data leakage.
\item Results from a large-scale study on data leakage in public notebooks.
\item Recommendations on process designs that prevent data leakage.
\end{itemize}
    
We share our tool and supplementary materials on GitHub.\footnote{https://github.com/malusamayo/leakage-analysis}


% \section{Old introduction}

% Will a promising machine learning model in experimentation work when deployed in the wild?
% This is often difficult to answer. There are many reasons why a model may perform well on test
% data, but not on operational data.
% Maybe the data collected for training is not representative enough of the operational data, producing a model that works for a different data distribution. 
% Maybe the model is overfitted to the test data, especially when test data is used for model selection.
% Maybe the model is exposed to the test data in the training stage, thus gaining an advantage it should not have.
% There are many pitfalls data scientists may fall into, 
% causing an over-optimistic estimate of various metrics of the final model, 
% and therefore over-confidence in how the model will perform in production.
% \cynote{add some descriptions about contract/model team}

% Among all potential issues, one of interest is leaking information about test data into the model training procedure, referred to as \textit{data leakage} in the literature.
% data leakage is often the result of using bad practices when writing machine learning code,
% ranging from obvious mistakes such as including test data in the training data,
% to more subtle ones that leak test data distribution information through preprocessing prior to training.



% In Fig.~\ref{fig:leak_acc}, we show an example where data leakage leads to over-optimistic test score.
% In this example, we generate synthetic data where both inputs and labels are random and independent (line 2-5).
% Therefore, any ML model should not perform significantly better than a random guess.
% However, due to a preprocessing leakage, where the feature selection step uses the test data (line 13),
% the model is no longer independent from test data.
% By selecting features that correlate better with test data, the biased test score (0.76) is much higher than expected.

% Despite explicit warnings from library developers~\cite{scikit, imblearn} and ML tutorials~\cite{alexisbcook_2021}, 
% data leakage problems are still surprisingly common in data science code.
% The results of our empirical study show that more than xx\% notebooks sampled from GitHub
% may have data leakage issues (Section \ref{sec:empirical-study}).
% Even many top Kaggle competition solutions inadvertently leak their test data,
% where the competitors already have limited access to it.
% Even though in many cases these issues may not result in significant evaluation bias,
% there are cases where these practices could have a significant negative effect.
% When beginners learn from these top notebooks in GitHub or Kaggle, 
% they may not realize that the code patterns that they follow are inherently problematic 
% and may apply them to other problems where it does make a difference (e.g., out of distribution predictions).
% Therefore, it would be useful if data leakage problems, just like any bugs or smells,
% could be highlighted during model development, before they are put into production.

% In this work, we develop an approach to automatically detect data leakage from source code via static analysis.
% We then use it to understand leakage problem in practice, 
% including an empirical study on hundreds of thousands of open-source data science notebooks and competition solutions.
% We discuss the impact of data leakage and recommend prevention measures.
% We formalize and implement our analysis in datalog, a popular language for declarative program analysis.




\section{Overfitting and Data Leakage in Machine Learning}\label{sec:overfitting}

Machine learning is the discipline of learning generalizable insights
from data, typically in the form of a learned function, called \textit{model}, that can make predictions
for unseen data (e.g., production data). Developers building models with machine learning techniques
usually follow an iterative and exploratory process~\cite{kery2018story} that is
commonly depicted as a pipeline of multiple steps with feedback loops, including activities such as
data collection, data cleaning, feature engineering, model training,
 model evaluation, and model deployment~\cite{microsoftSE4MLpaper}.
 
% \cynote{clarify that evaluation is only referring to test data}
 
In model development, there is always the risk that the trained model \textit{overfits} on
the data used for training~\cite{Russell1995ArtificialIA}---that is, it learns the patterns in the specific training
data but generalizes poorly to unseen data.
Therefore, it is customary to evaluate the accuracy of a model on 
data that was not previously used for training~\cite{Russell1995ArtificialIA}---the evaluation measures
to what degree the model predicts expected results for unseen data.
For the evaluation to provide a meaningful approximation of the model's accuracy in production settings, the unseen data needs to be representative of the distribution of real data encountered in production.


Overfitting can happen whenever insight is gained from data,
whether it is (a) a machine learning algorithm that is learning model parameters from
data or (b) a human looking at data to make decisions about how to process the data
or about what machine learning algorithm to use.
Most importantly, due to the iterative nature of model development, it is common to evaluate
 different variants of a model to see whether accuracy improves
with different decisions (e.g., different feature engineering, different
machine-learning algorithm, different hyperparameters; some of this
exploration may also be automated using AutoML approaches~\cite{He2021AutoMLAS}). If decisions are based on prior evaluation,
the data used in that evaluation influenced the training process and
the model may overfit on it.

In summary, if we evaluate the model on data that was used in any form 
(automated or manually, directly or indirectly) in the socio-technical process used for training the model, the 
evaluation result may be overly optimistic because the model may have overfit
on that data.
In a technical sense, we want a \textit{non-interference guarantee} in
which the process of training the model is entirely
independent of the data on which the model is evaluated.


\paragraph{Offline/Online Evaluation}
% \hl{
The model evaluation we discuss \linebreak above is usually executed offline \textit{before} model deployment.
Model developers could also conduct an online evaluation with production data \textit{after} their model is deployed. 
Typically offline evaluations are conducted to gain confidence in the model before deployment and to avoid exposing users to low-quality models in production, 
just like software developers rely on unit testing to identify software bugs rather than only relying on crash reports and bug reports from users in production.
% Though scores derived from online evaluation better represent reality, in many scenarios online evaluation is infeasible due to extra labeling efforts or lack of data.
% Therefore, model developers rely on offline evaluation to locate and fix potential issues before deployment,  
% just like software developers rely on unit testing to fix software bugs early in development.
% }

% \subsection{Data Science Pipelines}
% A typical data science project often has a pipeline structure:
% data is first collected, and then preprocessed.
% The prepared data is used for training and evaluation,
% which is an iterative process.
% \cynote{the evaluation is no longer unbiased if carried this way}.
% When the model satisfies various requirements, it is deployed in production,
% where it is tested against unseen/production data.

\paragraph{Training-Validation-Test Splits}

In many settings, labeled data that can be used for training or evaluation is limited and expensive to gather. Many data science projects start with a single dataset, from which separate subsets are used for training and evaluation.
The most common approach is to split data three ways into 
\textit{training data}, \textit{validation data}, and \textit{test data}.
Training data is used to develop the model and validation data is used
for preliminary evaluation during model development (including hyperparameter tuning), whereas test data should just be used once as a final unbiased evaluation of the final model.
Validation and test data seem similar and they are often used in the same type of evaluation functions in  machine learning APIs, but they serve fundamentally different purposes---validation data is used for decision making during model development and hence not suitable for an independent evaluation. 

The concepts of overfitting and the need to properly split data into these three sets to achieve unbiased evaluation results are universally covered in machine learning education and explained extensively in textbooks and course materials~\cite[e.g.,][]{Russell1995ArtificialIA, MLtextbook}.

% If all data is independent and from the same distribution, data is commonly split randomly into these three datasets.







% \subsection{Train-validation-test Splits}
% Usually, data scientists split their datasets into two parts: training data and test data. 
% They learn from training data to build models and later validate/test these models using test data.
% The main reason for the split is that in the learning procedure,
% the model is gradually overfitted to the data it is trained on.
% The score on training data, therefore, would be over-optimistic.
% The test data approximates the true score the model would get when it is applied to unseen data.

% In many cases, there is a third part: validation data. It is used for providing a less biased score in the training procedure while tuning hyperparameters.
% However, we still need a separate test data, since validation is no longer unbiased in the tuning process.
% Our discussion mainly focuses on leakage between training data and test data.
% \cynote{reason for this (we dont actually actively distinguish between test/validation in our leakage detection)}


\input{body/intro-example}


\paragraph{Data Leakage}
Despite the conceptual requirement to never make any decisions 
that influence the model based on data that is used for evaluating
the final model (i.e., noninterference of test data on model training), 
in practice, violations of this requirement are common and known as
\textit{data leakage} (because test data ``leaks'' into the training process)~\cite{burkov2020machine, kaufman2012leakage, DBLP:journals/corr/abs-2110-08339, deepchecks}. We target three forms of data leakage:

% In order to get an unbiased test score,
% data scientists need to make sure that 1) test data distribution is close to unseen data,
% and 2) test data is independent from the trained models.
% For the second requirement, the principle is that information of test data should not be used in any way in decision making of building a ML model. 
% This includes decisions made by ML algorithms and decisions made by humans. 
% Otherwise, there will be \textbf{data leakage} in the training procedure.
% The test data could be used in many ways to influence the training procedure. 
% Among them there are three major cases:

\begin{itemize}
    \item 
\textbf{Overlap Leakage:}
An obvious form of leakage occurs when some or all test data is directly used as input for training or hyper-parameter tuning. 
More subtly, leakage can occur when creating training data based on test data in the form of data augmentation or oversampling, as in Fig.~\ref{code:overlap_example}.
We call this type of leakage \textit{overlap leakage}, as rows of test data overlap with rows of training data. 

\item 
\textbf{Multi-Test Leakage:} 
If data is used repeatedly for evaluation, it is highly likely that
decisions are made based on that data, including algorithm selection, 
model selection, and hyperparameter tuning. For example, data scientists may have selected the model that works best on the data. Data used repeatedly in evaluation, as in Figure~\ref{code:multi_test_example},
can no longer be considered as unseen \textit{test} data, but should be considered as \textit{validation} data.
% Unfortunately, from an outside perspective we cannot always distinguish whether
% data is intended as validation or test data -- we report a leakage warn where data is used repeatedly in evaluations without separate test data used only once as 

  

\item 
\textbf{Preprocessing Leakage:} 
When training data and test data are preprocessed (transformed) together, 
test data sometimes influences the transformations of the training data.
For example, data could be normalized according to the largest and smallest values in both training and test data, rather than only based on values from training data.
Preprocessing leakage can occur in many transformations that consider multiple rows of the dataset,  
including feature selection (e.g., Fig.~\ref{fig:leak_acc}), normalizing data, projecting data with PCA, and vectorizing text data (e.g., Fig.~\ref{code:pre_processing_example}).
In many practical settings, training and test data have very similar distributions and preprocessing leakage has  only marginal influence on training data and hence the model; however, it is easy to construct examples where the mere knowledge about the distribution of test data can lead to substantial overfitting (see Fig.~\ref{fig:leak_acc}) and
 out-of-distribution predictions are particularly affected. 
%  In addition, it is a bad practice that violates the \textit{non-interference} requirement.
% These operations often leak distribution of test data, which is a more serious issue
% when there exists a significant difference between training data and test data distribution.
\end{itemize}

We target these forms of leakage because they are common sources of overconfident evaluation results, are discussed frequently both by practitioners and the literature~\cite{burkov2020machine, DBLP:journals/corr/abs-2110-08339}, and could be detected with static inspection of source code without understanding of the semantics of the data.
Other forms of leakage are beyond the scope of this paper, including \textit{label leakage} where unintended features in the data correlate with labels, leading to shortcut learning \cite{geirhos2020shortcut, kaufman2012leakage,burkov2020machine}; leakage from \textit{incorrect splits} of data when dependencies between rows exist, such as in time-series data~\cite{splits-aiops,burkov2020machine}---both of these forms of leakage require a deep understanding of the semantics of the data and are orthogonal to the three forms of data leakage we address.

    % \item Training data and test data are dependent. This often happens when the data is split in the wrong way or at the wrong point.
    % Sometimes the dataset itself may also contain duplicates or near-duplicates that cause dependency~\cite{Barz2020DoWT}. 
    
    % other factors:
    % test/deployment data distribution mismatch
    % misleading metric
    % label/target leakage

% In all these cases, model developers extract information from test data (intentionally or unintentionally), and use it to build a model, rendering model evaluations potentially unreliable. 
% That is, the learned model depends to some degree on the values of the test data, even though test data should serve solely as a way to obtain an unbiased evaluation of model performance.
% Otherwise, we will break the basic statistical assumption that test data is independent from the trained model,
% in which case it will no longer be a good approximation of unseen data.


==> body/2-approach.tex <==
\section{Approach}
\begin{figure}[t]
   \centering
  \includegraphics[width=\columnwidth]{images/approach-pic.pdf}
  \caption{Approach Overview.
  Our analysis first performs standard pointer analysis and data-flow analysis,
  and collects domain-specific information (dataset transformations, related-data, data-model mappings) from the results.
  Finally, leakage is detected using all the information collected.
}
  \label{fig:approach}
  \vspace{-1em}
\end{figure}

\input{body/approach-example}


\noindent We developed a static code analysis approach to detect different forms of data leakage. 
We analyze how data flows through notebook code and how it is used for training, validation, and testing.
To this end, we statically collect specific information needed to detect leakage (see Fig.~\ref{fig:approach}):
\begin{itemize}\item
\textbf{Dataset transformations.} In the preprocessing steps, transformations may leak information across rows, duplicate rows, or transform rows independently. 
Some of these transformations could contribute to preprocessing leakage or overlap leakage. 
Therefore, we need to track how datasets are processed. To this end, we label data-flow edges to track different kinds of dataset transformations.

\end{itemize}
\begin{itemize}\item
\textbf{Related-data relations.} To map data to models and detect overlap leakage, we need to understand whether datasets may have originated from the same rows in an original dataset. 
We track this with a related-data\emph{ relation} on top of our standard data-flow relations that tracks which two variables are related.

\end{itemize}
\begin{itemize}\item
\textbf{Data-model mappings}. To detect leakage, we need to identify the training/validation/test data for a given model. 
Here the key challenge is to differentiate validation and test data. 
We collect this information in data-model mappings, built on top of the related-data relations.

\end{itemize}
Once we have collected data flows (including data transformations and related-data relations) and data-model mappings, we can detect leakage by matching patterns over this information. In the remainder of this section, we explain each of these steps using a running example (Fig.~\ref{fig:approach_example}).


\subsection{Tracking Data Flows}

For all leakage detection, we need to identify how datasets and other computations relate to each other in the notebook. 
That is, we need to track how data may be repeatedly transformed and split, possibly by using information originally derived from other parts of the data, until it flows into training or evaluation functions of models. 
To this end, we perform standard data-flow analysis through assignments and method calls. In addition, we collect additional information about dataset transformations and related-data relations:


\input{body/datalog}

\subsubsection{Dataset transformations}
\label{sec:dataset-transform}

\label{h.dkl661gkybmp}
When tracking data flow, we are particularly looking for flows that are prone to leak information across multiple rows in a dataset or create new rows from old rows. 
The key insight is that transformations that remove rows or process data one row at a time are not problematic from a leakage perspective,
but transformations that process multiple rows together (as simple as counting or as complex as normalizing data by the largest value in a column) may cause leakage as rows may no longer be independent. 
In terms of typical concepts in functional programming, \textit{map}-like and \textit{filter}-like\footnote{
Technically, filter functions may change the length of a dataset and could leak information in the sense of non-interference. Pragmatically, we consider filter as unproblematic for data leakage, as filter is commonly used by data scientists for removing data points and therefore reporting this would not be very useful.}
transformations are okay, but \textit{reduce}-like transformations are suspicious.

To this end, our analysis labels 
(a) data-flow edges between datasets that perform computations independently on each row (map-like transformations) as \emph{map} edges and
(b) edges originating from datasets that perform computations across rows (reduce-like transformations) as \emph{reduce} edges. 
We manually label APIs in popular libraries (numpy, pandas, and sklearn) to identify those that perform computations per rows, 
such as \emph{fillna} (replaces missing values with the provided value) and those across multiple rows, 
such as \emph{numpy.mean} (computes a value based on multiple rows) and \emph{SelectPercentile.fit} (learns features from analyzing all rows). 
Notice that a \emph{reduce} edge may produce a single scalar value (such as calculating the mean of a column) which may be used subsequently in a map-like transformation (e.g., replacing missing values with that mean). 
Our analysis will later use this information to detect leaks when data flows through a \emph{reduce} edge.

In a similar fashion, we also identify transformations that duplicate rows (e.g., \emph{SMOTE.fit\_resample} from Fig.~\ref{code:overlap_example}) as \emph{duplicate} edges, 
which are potentially problematic because they can create dependencies between rows within a dataset, making random splits no longer produce independent datasets. 
% All three types of edges (map, reduce, and duplicate) are shown as inputs in Fig.~\ref{fig:rules}.

In our running example (Fig.~\ref{code:dataflow1}), we see a preprocessing operation that may introduce leaks: \emph{SelectPercentile.fit}, 
as it uses the distribution information of the input data. It corresponds to a \emph{reduce} edge from \emph{X\_0} to \emph{select}.
Operation \emph{SelectPercentile.transform}, on the other hand, corresponds to a \emph{map} edge from \emph{X\_0} to \emph{X}.



\subsubsection{Related-data relations}
\label{sec:related-data-rel}

\begin{figure}[t]
\begin{subfigure}[b]{0.3\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{images/split_a.pdf}
  \caption{}
  \label{fig:rel-data:a}
\end{subfigure}
\begin{subfigure}[b]{0.3\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{images/split_b.pdf}
  \caption{}
  \label{fig:rel-data:b}
\end{subfigure}
\begin{subfigure}[b]{0.3\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{images/split_c.pdf}
  \caption{}
  \label{fig:rel-data:c}
\end{subfigure}
\vspace{-1em}
\caption{Related-data relations are usually not transitive (a), except for duplicate edges (b) or map edges (c). Solid arrow edges are normal data-flow edges; dotted edges are related-data relations.
}
  \label{fig:rel-data}
  \vspace{-1em}
\end{figure}

\looseness=-1
In many steps for detecting leakage, we need to identify whether two datasets are related or independent. 
For example, to reason about repeated evaluations with test data (multi-test leakage), 
we need to understand whether the data used in two test locations
% \footnote{In the rest of the paper we use the term location to refer to program location in the notebook under analysis.}
are independent or somehow related. 
Technically, we establish a \emph{related-data relationship} to track whether two variables relate to each other (\textit{RelData} in Fig.~\ref{fig:rules}).
We consider two datasets as related (a) if they contain the same data, (b) if one is derived from the other, or (c) if they share rows from the same origin.

First, two datasets with a direct dataset flow (i.e., data-flow that only considers datasets) relation are considered as related (rule \textit{reldata/flow} in Fig.~\ref{fig:rules}). 
This is commonly the case when one dataset is a transformed version of another (e.g., Line 9 in our running example transforms \textit{X\_0} into \textit{X}) or simply assigned from one variable to another. 
Also, splitting a dataset creates multiple datasets that are each considered related to the original dataset (e.g., in Line 11 in our running example, \textit{X\_train} and \textit{X\_test} are both related to \textit{X}).
Our related-data relationship is reflexive and symmetric (rules \textit{reldata/ref} and \textit{reldata/sym} in Fig.~\ref{fig:rules}).

When two datasets are derived from the same original dataset, reasoning about their relationship is more complicated. 
In the common case that a dataset is split correctly into independent training and test sets, these two derived datasets should not be considered as related. 
However, when two datasets are derived from the same rows of an original source (e.g., two different ways of normalizing the entire dataset) they should be considered as related. 
Ideally, we would reason about transformations at the row level and consider datasets as related if their rows' origins in another dataset overlap, 
but corresponding dynamic analyses \cite{titian, newt, ramp} create runtime overhead and are difficult to adapt to our analysis. 
Instead, we approximate the most common patterns statically.

By default, we assume that two datasets derived from the same origin dataset are derived with a correct split and are hence considered as not related (Fig~\ref{fig:rel-data:a}). 
However, if we know that one of the datasets is derived with a map-like transformation (\textit{map edge} in Sec~\ref{sec:dataset-transform}) that dataset shares all rows with the original dataset and is not involved in a split. 
Hence, we consider that dataset as related to all other datasets derived from the same origin (Fig.~\ref{fig:rel-data:b}; rule \textit{reldata/map} in Fig.~\ref{fig:rules}). 
Furthermore, if the origin dataset contains dependent rows (e.g., from a data augmentation step), we assume that derived datasets are also related, as splits are unlikely to maintain independence. 
Hence, we consider all datasets derived from an origin where data was produced (directly or indirectly) through a duplicate edge (see Sec~\ref{sec:dataset-transform}) as related (Fig~\ref{fig:rel-data:c}; rule \textit{reldata/dup} in Fig.~\ref{fig:rules}). 
\looseness=-1

Note that our three heuristics approximate a more accurate dynamic analysis, but cannot cover all cases. 
For example, our heuristic would identify a split with overlapping rows (\textit{a, b = o[:100], o[50:]}) as independent, but those mistakes are very rare. 
We consider that the cost of increased false positives or more expensive dynamic analysis outweigh the benefits of detecting such very rare cases. 
As we will show in our evaluation in Section~\ref{sec:empirical-study}, our heuristics capture the relationships found in common notebooks to achieve relatively accurate leakage detection.




\subsection{Data-Model Mappings}
\label{sec:model-data}

While data-flow analysis tracks how data is transformed and moves through the notebook, 
we can only identify whether data is training data, validation data, or test data by determining how it is eventually used.

As a first step, we identify program locations where (usually preprocessed) data is used for training, validation, and testing. 
We identify those locations simply by finding API calls in the notebook that are typically used for training and evaluation purposes, such as the \textit{fit} and \textit{predict} functions in \textit{sklearn}'s APIs.
We later trace back the source of the data used in these APIs to processing steps and original datasets using standard data-flow analysis.

\looseness=-1
While training data can be identified with distinct function calls, distinguishing between validation and test data is conceptually challenging because both are used with the same APIs (e.g., predict). 
We cannot reliably infer whether a data scientist intends to use data for validation or testing purely based on notebook code---this is a challenge even for human experts who may need to rely on context clues or documentation. 
We therefore rely on a simple heuristic that considers data that is used repeatedly in evaluation as validation data and all data that is used only once in evaluation as test data.
We consider data to be evaluated repeatedly if its location is within a loop or if two locations are connected to evaluate the same or related data as per our data-flow analysis (i.e., variables in both locations are connected through the related-data relation from Sec.~\ref{sec:related-data-rel}).

Finally, we group each training dataset with the corresponding validation and test datasets that relate to the same model. 
We use standard data-flow analysis to identify which call locations share the same target object. To account for possible repeated training of the same model object, 
we always group training data with all subsequent validation and test data, until the next training data is identified. 
In the end, we derive a series of model-data tuples (\textit{ModelData} in Fig.~\ref{fig:rules}),
% : (model, training\_data, validation\_data\_set, tes\_data\_set),
where the same training data might correspond to zero or multiple validation/test datasets. 
In our example (Fig.~\ref{code:dataflow1}), we show two model-data tuples based on this heuristic: (\textit{lr}, \textit{X\_train}, \{\textit{X\_test}\}, $\varnothing$) and (\textit{ridge}, \textit{X}, \{\textit{X\_test}\}, $\varnothing$).




\subsection{Leakage Detection}
After collecting the above information, identifying leakage is performed through pattern matching:

\begin{itemize}\item
\looseness=-1
To detect multi-test leakage, we check for a given model whether there exists at least one piece of test data. 
Note that `test data' evaluated multiple times will already be identified as validation data in our analysis (see Sec.~\ref{sec:model-data}). 
If for all models, there is no test data but only validation data detected, we report multi-test leakage (rule \textit{leak/multi} in Fig.~\ref{fig:rules}).

\item
To detect overlap leakage, we check for a given model \linebreak whether training data and test/validation data\footnote{
Note that for overlap/preprocessing leakage, we do not distinguish between test and validation data. Leakage between training data and validation data is still problematic, as it defeats the purpose of validation data (i.e., providing independent validation during model development).}
are related. 
Note that there might be multiple test/validation data in a single model-data tuple (see Sec.~\ref{sec:model-data} for how we derive the tuple). 
Therefore, for a given trained model, we only report overlap leakage when all of its test/validation data overlaps with the training data  (rule \textit{leak/overlap} in Fig.~\ref{fig:rules}).

\item
To detect preprocessing leakage, we check whether training data contains information from test/validation data through preprocessing (\emph{reduce} edges). 
If training data uses reduced information from test/validation data (or datasets that are related to test/validation data), we will report a case of preprocessing leakage  (rule \textit{leak/pre} in Fig.~\ref{fig:rules}).

\end{itemize}

In our example, we could find a path from \textit{X} to \textit{X\_train} and a path from \textit{X\_0} to \textit{X\_test} (see Fig.~\ref{fig:dataflow}). 
As \textit{X} contains reduced information from \textit{X\_0}, which is related to \textit{X\_test}, 
we establish that test data information is leaked into training data, and there is a preprocessing leakage.
Next, because \textit{X} is related to \textit{X\_test} (as \textit{X\_test} is transformed from \textit{X}), 
there is an overlap leakage when we evaluate the second model \textit{ridge}.
Finally, the two trained models share the same test data (\textit{X\_test}), which we will identify as validation data. 
Because there is no independent test data used in the final evaluation, we conclude that there is also a multi-test leakage.

In the fixed version of our example (see Fig.~\ref{code:dataflow2}), we see that the two model-data tuples are changed to (\textit{lr}, \textit{X\_train}, \{\textit{X\_test}\}, \{\textit{X\_test\_new}\}) and $(\textit{ridge}, \textit{X}, \{\textit{X\_test}\}, \{\textit{X\_test\_new}\})$ and hence: (1) models no longer contain information from \textit{X\_test}, as the reduced information only comes from \textit{X\_train} (see Fig.~\ref{fig:dataflow2}), eliminating the preprocessing leakage, (2) in all tuples, training data and test/validation data are no longer related, eliminating the overlap leakage, and (3) there is independent test data \textit{X\_test\_new} that is evaluated only once, eliminating the multi-test leakage.


\subsection{Implementation}
To make our analysis easy to extend and modify, our implementation uses \textit{datalog}, a language commonly used in declarative program analysis~\cite{smaragdakis2015pointer, bravenboer2009strictly}. 
Our two-phase implementation first transforms Python code into datalog facts as an intermediate representation and then analyzes these facts to generate leakage detection results. Our analysis design is similar to \emph{doop}~\cite{bravenboer2009strictly}, a popular Java program analysis framework.

% \paragraph{Fact Generation}
In the front end, we generate datalog facts that can be easily analyzed subsequently. Specifically, we
translate complex language structures into simpler ones,
translate assignments (both variables and fields) to static single assignment form, which ensures that subsequent analyses are flow-sensitive,
and match method invocations with signatures.
% \end{itemize}
To identify datasets and targets of method invocations, we perform type inference with the off-the-shelf type inference engine \textit{pyright}~\cite{pyright}. 


% \paragraph{Datalog Analysis} 
Based on initial datalog facts, we compute additional facts for the relations (e.g., \emph{RelData}, \emph{ModelData}) described above and subsequently detect data leakage using datalog queries.
We implement a standard Anderson-style 2-call-site-sensitive pointer analysis similar to \emph{doop}, with special treatment of common language features (e.g., lists and global variables). 
The data-flow analysis is built on pointer analysis and also follows standard implementations.

% \paragraph{API Specifications}
Our analysis requires specifications of data science APIs. Specifications are mainly used to provide domain knowledge (e.g., which APIs are used for training/testing, which APIs behave \textit{reduce}-like).
Our current implementation supports three machine learning libraries -- \textit{sklearn}, \textit{keras}, and \textit{pytorch} -- and two libraries commonly used for data transformations -- \textit{pandas} and \textit{numpy}. 
We went through the official documentation of these libraries to find APIs that perform data transformations and
APIs that perform supervised learning. %, as leakage in the unsupervised learning setting is out of scope.
% \hl{Details of API specifications are provided in the supplementary materials.}
Our analysis can be easily extended to other libraries by providing their specifications.


% \begin{table}[t]
% \begin{tabular}{llllll}
% \toprule
% \#API & numpy & pandas & sklearn & keras & pytorch \\
% \midrule
%  &  &  &  & &  \\
% \bottomrule
% \end{tabular}
% \caption{We label xxx APIs from 5 popular data science libraries.}
% \label{tab:api}
% \end{table}



% We developed an approach based on static code analysis to detect different forms of data leakage. 
% % Our approach decomposes the problem into multiple steps:
% Specifically, we analyze how data flows through the notebook code and is used for training, validation, and testing. 
% There are multiple more nuanced pieces of information we need to collect to determine leakage.

% \begin{itemize}
%     \item For overlap leakage, we need to identify whether data used in training or validation and testing may have originated from the same rows in an original dataset. 
%     We track this with an overlap relation on top of our standard data-flow relations that tracks which two variables may contain overlapping rows or data derived from overlapping rows.
    
%     \item For multi-test leakage, we need to identify whether data is used repeatedly in evaluations. 
%     Here the key challenges are tracking how data is used for evaluating one or multiple models and how to differentiate validation and test data. 
%     We collect this information in data-model mappings.
    
%     \item For preprocessing leakage, we need to track how data is processed and which of these processing steps may leak information across rows. 
%     To this end, we collect additional information on dataflow edges to identify edges that potentially leak data, which we call reduce edges.
% \end{itemize}
% Once we have collected data flows (with additional information), overlap relations, and data-model mappings, we can detect leaks by matching patterns over these information. In the remainder of this section, we explain each of these steps, using a running example (Fig.~\ref{fig:ex_analysis}).

% % (see Figure~\ref{fig:approach}):
% % Given an input program,
% % our analysis first identifies program locations where data is used for model training and testing (\textit{model-data identification}) and where
% % operations are used for data processing that could leak information across rows (\textit{leakage source identification}).
% % Then for each data pair of a model, our analysis tracks their relevant information-flow and analyzes whether different datasets may overlap (\textit{overlap analysis}).
% % Finally, our analysis uses all this information to determine whether there is potential leakage in the input program (\textit{leakage detection}). 

% Note that we intentionally designed a static analysis approach rather than a dynamic analysis approach.
% Although a dynamic analysis would allow more precise tracking of individual rows of data, we selected a static approach because 
% (1) it is lightweight, faster, and does not produce runtime overhead in already computationally expensive executions,
% and (2) it allows us to more easily analyze a wide range of public notebooks (that are often challenging to reproduce~\cite{pimentel2019large}).
% Adopting a static analysis approach allowed us to perform the large scale study with thousands of diverse notebooks that we used for evaluation (Section \ref{sec:empirical-study}).

% % On the other hand, there are many unique challenges for developing a static analysis to detect data leakage.
% % It is hard to determine relations between datasets statically (e.g., whether two datasets overlaps).
% % Locating and grouping train/validation/test sites accurately is also non-trivial.


% % In other words, we need to identify and analyze
% % \begin{enumerate}
% %     \item the sites of training data, test data, and risky operations

% %     \item overlaps and flows between different variables.
% % \end{enumerate}

% % For the first requirement, we match method calls with known APIs with corresponding functionalities.   
% % For the second one, we rely on a custom static analysis that approximates the actual overlap and dynamic flow between variables.

% \subsection{Tracking Data Flows}
% For all leakage detection, we need to identify how datasets and other computations relate to each other in the notebook. 
% That is, we need to track how data may be repeatedly transformed and split, possibly by using information originally derived from other parts of the data, until it flows into training or evaluation functions of models. 
% To this end, we perform standard data flow analysis through assignments and method calls 
% % (standard def-use analysis, using models for common APIs to improve accuracy without analyzing code of external libraries) 
% and collect additional information about the kinds of flows, relations among variables (reduce/flatmap edges, dataset/equivalent flows), and overlap relations.

% \subsubsection{Reduce/flatmap edges}
% While tracking data flow, we are particularly looking for flows that are prone to leak information across multiple rows in a dataset or create new rows from old rows. 
% The key insight is that transformations that remove rows or process data one row at a time are not problematic from a leakage perspective, 
% but transformations that process multiple rows together (as simple as counting or as complex as normalizing data by the largest value in any row) or create new rows based on existing rows (e.g., in oversampling) may cause leakage as rows may no longer be independent. 
% In terms of typical concepts in functional programming, filter-like and map-like transformations are okay, but reduce-like and flatmap-like transformations are suspicious. 

% To this end, our analysis labels dataflow edges that come from possibly problematic APIs as reduce/flatmap edges. 
% We manually label APIs in popular libraries (e.g., numpy, pandas, and sklearn) to identify those that perform computations across multiple rows, such as \textit{numpy.mean} and \textit{SelectPercentile.fit}.
% Notice that a reduce edge may produce a single scalar value (such as taking the max of a column) and that this value may be used in a map-like transformation later (e.g., normalizing to that max).
% Our analysis will later catch this as a problematic leak since it will identify a dataflow through a reduce edge.

% In our example (Fig.~\ref{code:dataflow1}),
% we could find a preprocessing operation that may introduce leaks: \textit{SelectPercentile.fit}, 
% as it uses the distribution information of input data. 
% It corresponds to a \textit{reduce} edge from \textit{X\_0} to \textit{select}. 

% \begin{figure}
% \begin{subfigure}[b]{0.3\columnwidth}
%   \centering
%   \includegraphics[width=\columnwidth]{images/split_a.pdf}
%   \caption{}
% \end{subfigure}
% \begin{subfigure}[b]{0.3\columnwidth}
%   \centering
%   \includegraphics[width=\columnwidth]{images/split_b.pdf}
%   \caption{}
% \end{subfigure}
% \begin{subfigure}[b]{0.3\columnwidth}
%   \centering
%   \includegraphics[width=\columnwidth]{images/split_c.pdf}
%   \caption{}
% \end{subfigure}
% \caption{Related-data relations are usually not transitive (a), except for duplicate edges (b) or map edges (c). (Solid arrow edges are normal data flow edges; dotted edges are related-data relations.)
% }
%   \label{fig:mapreduce}
% \end{figure}


% \begin{figure}
% \begin{subfigure}[b]{\columnwidth}
%   \centering
%   \includegraphics[width=\columnwidth]{images/mapreduce.pdf}
%   \end{subfigure}

% \begin{subfigure}[b]{\columnwidth}
% \begin{lstlisting}[language=Python]
% x = input() # read input to an Series object
% m = x.mean() # reduce
% x = x.fillna(m) #map
% x = x.loc[x >= 0] # filter
% // x = oversampler.fit_sample(x) # flatmap
% \end{lstlisting}
% \end{subfigure}

% \caption{Common data processing operations can be classified into four categories. 
% Reduce/flatmap operations could be potential leakage sources if they are performed before train/test splits.
% }
%   \label{fig:mapreduce}
% \end{figure}


% \subsubsection{Overlap relations}
% [repeat motivation for overlap relations]
% \cynote{dataset independent/related -> tracking origins}

% For overlap relations, we want to track whether two datasets have rows originating from the same rows in the original dataset.
% Intuitively, a typical case would be when one dataset is derived from another, two datasets overlap.
% Therefore, it is common for two datasets to overlap in the preprocessing stage.
% Dynamically, this could be achieved through record-level provenance tracking (e.g., Titian~\cite{titian} or RAMP~\cite{ramp}),
% where for a given row in the output dataset, they trace back to input rows that are transformed into it.
% For a map operation, the mapping would be one-to-one, while a reduce operation would have a many-to-one mapping.

% Statically, we approximate this through tracking how datasets are transformed.
% For a given dataset, we trace back through its flow path to find its ancestor datasets that are later transformed into it.
% In this case, we know that they have overlapping origins.
% Overlap relation is usually not transitive (e.g., when two datasets $a$ and $b$ both overlap with $c$, they might still not overlap with each other, as their respective overlapping origins could be disjoint),
% except when we have two datasets that share exactly the same original rows (which we refer to as equivalent datasets).
% In that case, any datasets that overlap with one of the two would also overlap with the other.
% We could track dataset equivalence through checking whether transformation between two datasets only uses map-like operations. 

% Additionally, a special case of overlapping happens when a dataset split is performed after flatmap operations. 
% The resulting split datasets are likely to overlap with each other, as they might contain duplicated rows from the original dataset.

% To derive overlap relations, we label APIs that transforms datasets, 
% such as \textit{train\_test\_split} and \textit{SelectPercentile.transform}.
% Edges that come from these APIs are marked as `dataset' edges.
% For those map-like APIs, we also mark their edges as `equivalent' edges.
% When two datasets could be connected using only these edges, we could confirm that one of them is transformed into the other.

% In the example in Figure~\ref{fig:dataflow}, we see that $X\_0$ and $X\_test$ overlap because there $X\_test$ is transformed from $X\_0$. 
% Similarly, $X\_0$ and $X\_train$, $X\_0$ and $X$ also overlap.


% \subsection{Data-Model Mappings}
% \label{sec:model-data}
% While dataflow analysis tracks how data is transformed and moving through the notebook, we can only identify what data is training, validation, and test data by how it is eventually used.

% As a first step, we identify program locations where (usually preprocessed) data is used for training, validation, and testing. 
% We identify those locations simply by finding API calls in the notebook that are typically used for training and evaluation purposes, such as the fit and predict functions for sklearn models. 
% We will later trace back the source of the data used in this API to processing steps and original datasets using standard dataflow analysis.

% While training data can be identified with distinct function calls, distinguishing between validation and test data is conceptually challenging, 
% since both are used with the same APIs (e.g., predict). We cannot reliably infer whether a data scientist intends to use data for validation or testing purely on the notebooks code -- 
% this is a challenge even for human experts who may need to rely on context clues or documentation. 
% We therefore rely on a simple heuristic that considers data that is used repeatedly in evaluations as validation data and all data that is used only once as test data. 
% We consider data to be used repeatedly if the location is within a loop or if two locations are connected to use the same or overlapping data as per our dataflow analysis. 

% Finally, we group each training location with the corresponding validation, and test locations that relate to the same model. 
% We use a simple dataflow analysis identifying which call locations share the same target object. 
% To account for possible repeated training of the same model object, 
% we always group a training location with all subsequent validation and test locations, 
% until the next training location. 
% In the example (Fig. 4a), we show two pairs of data data based on this heuristic: (X\_train, X\_test) and (X, X\_test)



% % \subsection{Pointer Analysis and Information-Flow Analysis}
% % To detect data leakage, we build standard pointer and information-flow analyses,
% % which other domain-specific analyses rely on.
% % They are useful for tracking whether two datasets may have shared records (i.e., overlaps), 
% % or whether one model depends on the other.

% % Later in overlap analysis, we need to distinguish between datasets and other variables and relations between different datasets (e.g., whether two datasets contain exactly the same data points).
% % Therefore, our custom analysis also extends the traditional information-flow graph with edge tags, which contain more granular information related to input datasets.
% % Specifically, we associate edges with two types of tags: (1) when one dataset flows to another dataset we tag the edge with `data', and (2) when one dataset flows to another dataset, and the operation is known to keep the same data records (i.e., it is not removing or adding new ones),
% % we tag its corresponding flow edge with `equivalent'.
% % Two datasets are equivalent if they contain same data records (id), even if the data records themselves may be transformed. 
% % For example, when a dataset is processed and renamed, the two contain the same data records, hence we consider them as equivalent.

% % In our example, the resulting information-flow graph is shown in Fig.~\ref{fig:dataflow}. 
% % In the graph, there are three \textit{data} edges that result from two operations: \textit{SelectPercentile.transform} and \textit{train\_test\_split}. 
% % The first operation also guarantees that the input dataset and the returned dataset are equivalent.


% % \subsection{Overlap Analysis}
% % In order to detect whether training data and test data overlap (which leads to overlap leakage),
% % we need to analyze whether any given two datasets may overlap.
% % Unfortunately, the precise information about dataset overlapping is inherently impossible to track statically.
% % Therefore, we use several heuristics to develop an approximation.

% % First, if one of the datasets flows into the other, it is very likely that they overlap. 
% % A typical example is when a new dataset comes from splitting an old one,
% % where the new dataset overlaps with the old one.
% % Second, when two datasets are equivalent, and one overlaps with a third dataset, the other one also overlaps with the third dataset.
% % Finally, when two datasets are derived from the same dataset, they are likely to overlap with each other if some operations introduce extra redundancy in the split dataset (e.g., oversampling).
% % % or 2) they are not guaranteed to come from non-overlapping splits.

% % We summarize our heuristics as below:
% % \begin{enumerate}
% %     \item Suppose that $x, y, z, a, b$ are all datasets.
% %     \item If there is a data path from $x$ to $y$ in the flow graph, then $x$ and $y$ \textit{overlap}.
% %     \item If there is an equivalence path from $x$ to $y$ in the flow graph, and $x$ and $z$ \textit{overlap}, then $y$ and $z$ \textit{overlap}.
% %     \item If there is an edge from $a$ to $b$, where redundancy is introduced, and there are data paths from $b$ to $x$ and $y$ respectively, then $x$ and $y$ \textit{overlap}.
% % \end{enumerate}


% % \subsection{Model-Data Identification}
% % \label{sec:model-data}
% % In this stage, we aim to identify all model-data pairs and separate them into training/validation/test data.
% % We rely on API specifications to find potential training/validation/test locations.
% % The main challenge  is that in many cases it is hard to 
% % distinguish between validation and test data, as the APIs they are fed into
% % are often the same.
% % Therefore, we rely on a single heuristic to find validation data: 

% % \textit{When the same data $x$ is evaluated multiple times (either in a loop or across different models), 
% % it is likely to be validation data.}

% % This heuristic is also extended to the case of overlapping data, where two pieces of evaluation data overlap.
% % In this case, we treat both of them as validation data.

% % After identifying individual model-data pairs, we need to find the corresponding training site for each test site.
% % This heuristic keeps the nearest training location where the trained model flows to the test model,
% % as all the data used before is cleared by the last training step.
% % In the example (Fig.~\ref{code:dataflow1}), we show two pairs of data data based on this heuristic:
% % (\textit{X\_train}, \textit{X\_test}) and (\textit{X}, \textit{X\_test}).

% % \subsection{Leakage Source Identification}


% % The last ingredient to our leakage detection is identification of potential leakage sources.
% % As discussed before, there are many operations that may lead to data leakage.
% % Our approach focuses on two kinds: 1) operations that over-sample/augment data,
% % and 2) operations that transform data with cross-sample information.
% % These operations risk leaking test data information to training data 
% % if they are performed before a data split.

% % From a functional perspective, preprocessing operations can be classified into
% % four types.
% % There are operations that behave similar to \textit{map}, where each data point is transformed independently and could be fully paralleled. 
% % Type conversion for data columns would be a typical example (see Fig.~\ref{fig:mapreduce}).
% % There are also operations that behave similar to \textit{reduce}, where data points are aggregated for extracting information (e.g., feature selection).
% % Lastly, there are operations that behave like \textit{filter} or \textit{flatmap}, where data points are removed or added.
% % We are mainly concerned about \textit{reduce} and \textit{flatmap} operations, 
% % as they make data points in the dataset no longer independent from each other.
% % This results in the split train/test data no longer being independent either.

% % Similar to training/validation/test sites, these risky operations are identified based on API specifications.
% % In our example (Fig.~\ref{code:dataflow1}),
% % we could locate a preprocessing point that may introduce leaks: \textit{SelectPercentile.fit}, 
% % uses the distribution information of input data. 
% % It corresponds to a \textit{reduce} operation, which connects a pair of source variable and target variable 
% % (\textit{X\_0} and \textit{select} in this case). 


% % % Method specifications are also used to cache information flow within the APIs, 
% % % such that the analysis could be performed within current module.

% % % In this stage, we produce three types of basic facts:
% % % \textit{TrainingData}, \textit{TestData}, \textit{ValData}.
% % % Their first arguments match the model they are trained/tested on,
% % % and their second arguments are the corresponding variable names.


% \subsection{Leakage Detection}
% After collecting these information, we could detect leakage through pattern matching:

% \begin{itemize}
%     \item To detect multi-test leakage, we check whether these exists at least one piece of test data. 
%     Note that `test data' evaluated multiple times will be identified as validation data in our analysis (see Section~\ref{sec:model-data}).
%     If there is no test data but only validation data detected, we reported multi-test leakage.
    
%     \item To detect overlap leakage, we check whether training data and test data overlap.
%     Note that the same training data may correspond to multiple pieces of test data. 
%     Therefore, for a given trained model, we only report overlap leakage when all of its test data overlaps with the training data.

%     \item To detect preprocessing leakage, we check whether training data contains information from test data through preprocessing (reduce edges).
%     If training data uses reduced information from test data (or datasets that overlap with test data), we will report a case of preprocessing leakage.
    
% \end{itemize}


% % Specifically, we check whether there exists
% % \begin{enumerate}
% %     \item a pair of variables (\textit{des, src}) that is connected by a reduce edge,
% %     \item a path from the \textit{des} variable to the training data, and
% %     \item overlap between \textit{src} and test data.
% % \end{enumerate}
% % When test data and \textit{src} overlap, the extracted variable (\textit{des}) is likely to contain information from test data. 
% % If it flows to training data, then test data is likely to be leaked.



% In our example, we could find a path from \textit{X} to \textit{train} and a path from \textit{X\_0} to \textit{test} (see Figure~\ref{fig:dataflow}). 
% As \textit{X} contains extra information from \textit{X\_0}, a super-set of \textit{test}, 
% we establish that test data information is leaked into training data, and there is a preprocessing leakage.

% Next, it is easy to determine that $X$ overlaps with $X\_test$ (as there is a flow between them in the graph), causing a leakage when
% we evaluate the second model $ridge$.
% Finally, the two data pairs (bounded by blue boxes in Fig.~\ref{fig:dataflow}) share the same test data,
% but no independent test data is used for final evaluation, which biases the test score of the final model.
% Therefore, we conclude that the code also contains a multi-test leakage.

% After fixing the code (see Fig.~\ref{code:dataflow2}), we see that
% \begin{enumerate}
%     \item $X\_train$ no longer contains information from $X\_test$, as the reduced information only comes from $X\_train\_0$
%     \item There is no overlap between any pairs of training data and test data.
%     \item There is an independent test set $X\_test\_new\_0$ that is used only once.
% \end{enumerate}


% \input{body/datalog}

% \subsection{Implementation}
% To make our analysis easy to extend and modify, our implementation is based on datalog,
% a language commonly used in declarative program analysis~\cite{bravenboer2009strictly}.
% Our two-phase implementation first transforms python code to an intermediate representation (IR) (datalog facts) and then analyzes these facts to generate leakage detection results.

% \paragraph{Fact Generation}
% In the front end, our goal is to generate facts that can be easily analyzed by model developers.
% Therefore, we need to
% \begin{enumerate}
%     \item translate complex language structures to simpler ones
%     \item translate assignments (both variables and fields) to static single assignment (SSA) form, which ensures that subsequent analyses are flow-sensitive
%     \item match method invocations with signatures
%     % , which is particularly challenging due to Python's dynamic typing
% \end{enumerate}

% To achieve this, we perform three passes over the input Python code. 
% The first pass translates the original Python code to an intermediate representation, where complex language constructs are translated to simpler ones in SSA form. 
% Conceptually, our IR is to Python what Shimple~\cite{soot} is to Java.
% The second pass generates type information using an off-the-shelf type inference engine called pyright~\cite{pyright},
% which is also used in the third pass to translate the IR to basic facts that can be easily processed by a datalog analysis engine. 
% The interface is similar to doop, a popular Java program analysis framework~\cite{bravenboer2009strictly}.

% \paragraph{Datalog Analysis}

% In the back end analysis, our goal is to detect data leakage from the program (in the form of datalog facts).

% % In Figure~\ref{fig:analysis}, we present our core analysis in datalog.
% We implement a standard Anderson-style 2-call-site-sensitive pointer analysis similar to doop, 
% with special treatment of realistic language features (e.g., lists and global variables).
% The information-flow analysis is built upon pointer analysis and also follows standard implementations.
% Our core datalog specifications are provided in the supplementary materials.

% \paragraph{API Specifications}
% Our analysis requires specifications of common data science APIs.
% They are mainly used to provide domain knowledge (e.g., which APIs are used for training/testing, which APIs behave like a \textit{reduce} or \textit{flatmap} operation).
% They are also useful for caching information flow within the APIs (i.e., how information of arguments propagates to returned variables).

% Our current implementation supports three learning libraries: sklearn, keras, and pytorch, 
% and also two libraries commonly used for data transformations: pandas and numpy.
% Our analysis can be easily extended to code using other libraries once their specifications are provided.


% \paragraph{User Interface}
% In our evaluation, we need to manually check the accuracy of the analysis results and also show
% the results to potential users.
% We built a simple user interface to facilitate both processes.
% The interface indicates the locations of training/test data and the potential leakage detected (see Figure~\ref{}).


==> body/3-evaluation.tex <==
%!TEX root = ../main.tex


\section{Evaluation}
We first evaluate the accuracy of our analysis, that is, its ability to find actual leakage and to avoid false alarms:
\begin{itemize}
    \item \textbf{RQ1}: \textit{How accurate are the results of our analysis?} 
\end{itemize}

To ensure that our analysis can be used in an interactive or continuous integration setting during  model development, we also evaluate  efficiency in terms of running time:
\begin{itemize}
    \item \textbf{RQ2}: \textit{How efficient is our analysis?} 
\end{itemize}


Finally, after establishing accuracy and efficiency, we use our analysis to study test-train leakage in a large corpus of notebooks, exploring common forms and sources of leakage. We will show that leakage is common across different types of notebooks. In addition, leakage often manifests itself in nontrivial data flows in notebooks, in forms that can be tedious or even difficult to detect manually, providing strong, albeit indirect evidence for the usefulness of our automated detection:
\begin{itemize}
    \item \textbf{RQ3}: \textit{How prevalent is data leakage in public notebooks?}% How frequent are they in beginner's and expert's code? And in the context of competitions?} 
    \item \textbf{RQ4}: \textit{What do typical leakage issues look like?}% How complex are the notebooks containing leakage?} 
\end{itemize}


\subsection{Research Design}
We evaluate all four research questions with a corpus of public data science code in Jupyter notebooks. For different research questions, we use different subsets of this corpus.

\subsubsection*{Corpus of notebooks with data science code.}
To answer our research questions, we curate a large corpus of public notebooks with data science code. 
Specifically, we collect Jupyter notebooks from GitHub and Kaggle.
GitHub is a common platform for storing data science code for a range of purposes, from hobby and educational projects, to research projects and tutorials, to production systems. Kaggle is a common platform for data science competitions where users can submit notebooks as solutions to competition problems.
We purposely selected code in notebooks, rather than arbitrary Python files, 
because notebooks are the primary environment for developing data science code~\cite{perkel2018jupyter}.


For GitHub, we collected \emph{all} notebooks from GitHub repositories created in September 2021 (strictly independent from all notebooks from earlier periods used during development of our analysis). Specifically, we used the GitHub search API to identify repositories with notebook code and partitioned the search space to collect \emph{all} \numprint{81026}~repositories. By selecting all notebooks from a recent time period, we get a full and representative sample of the different kinds of notebooks published on GitHub. We collected a total of \numprint{280994}~notebooks this way.

For Kaggle, we selected a smaller and more targeted notebook population, 
collecting notebooks from two popular competitions, \textit{titanic} and \textit{housing} \cite{titanic, housing}. 
For each competition, we collect the 200 notebooks with the most votes and the 200 most recent notebooks, as of April 12, 2022.
% \hl{
We selected these competitions, because they use tabular data and require significant preprocessing effort. 
We use this corpus to understand leakage issues among typical competition solutions that are prone to data leakage. 
They are not necessarily representative of all competition solutions on Kaggle.
% }
% , discarding duplicates.

We further filter these notebooks to include only those that use the machine learning libraries supported by our current implementation (\emph{sklearn}, \emph{keras}, and \emph{pytorch}). 
The discarded notebooks either only use not-yet-supported libraries such as \emph{tensorflow} or do not train any models. This leaves us with \numprint{107603} GitHub notebooks and \numprint{108273} in our corpus overall. In Table~\ref{tab:leakage}, we show descriptive statistics of our final corpus.

\begin{table*}[t]
\small
\begin{tabular}{lllllllll}
\toprule
Dataset & \#notebooks & LoC & \#stars & Preprocessing Leakage & Overlap Leakage & Multi-test Leakage & Any Leakage  \\
\midrule
GitHub (all)  & \numprint{107603} & 410  & 1.1 & 12.3 & 6.5 & 18.5 & 29.6 \\
GitHub (popular) & \numprint{920} & 378  & 95.2 & 4.9 & 5.2 & 15.9 & 20.9 \\
GitHub (tutorials) & \numprint{1157} & 584  & 4.2 & 3.9 & 2.9 & 11.3 & 16.2 \\
GitHub (assignments)& \numprint{7576} & 559  & 0.6 & 13.9 & 7.4 & 22.0 & 33.0 \\
Kaggle (top)  & 312 & 851 & - & 56.1 & N/A & N/A & N/A \\
Kaggle (recent)& 358 & 504 & - & 55.8  & N/A & N/A & N/A \\
\bottomrule
\end{tabular}
\caption{\small Data Leakage Distribution. LoC is the average number of lines of code across all notebooks in the group.
Number of stars is based on the repository that these notebooks reside in and is also averaged. 
We show the percentage of notebooks for which we report each leakage type. For Kaggle notebooks, we only track preprocessing leakage because the other two are infeasible in this setting (marked as N/A in the table).}
\label{tab:leakage}
\vspace{-1.5em}
\end{table*}


\subsubsection*{Analyzing accuracy (RQ1).}
Establishing ground truth for data leakage is challenging and we are not aware of existing datasets.
To evaluate the accuracy of our analysis, we measure both false positives and false negatives on a sample of notebooks for which we manually establish ground truth. 
Due to the substantial manual effort involved, we perform the analysis on 100 randomly sampled notebooks from our GitHub corpus (which yields an 8\,\% error margin with a confidence level of 95\,\%)~\cite{samplesize}.

One author manually labeled these 100 notebooks looking for leakage issues and then compared manual labels with the analysis results.
For all notebooks where the manual labels and analysis results disagreed,
the author sought the expert opinion of a second author (a trained data scientist). Together they discussed the issue to determine whether the notebook contained leakage, correcting the ground truth label if needed. 
This correction was needed in 7 notebooks, which were incorrectly labeled initially, arguably indicating that manual checking of data leakage is
non-trivial and error-prone, even for experts. 
Overall our process balances labeling effort and confidence in the ground truth.
% -- note that our approach does not detect cases where both manual label and analysis agree on the wrong outcome, but we consider those cases unlikely.

\looseness=-1
As per our manually established ground truth, 40 of the 100 notebooks contained at least one form of leakage -- 20 with preprocessing leakage, 8 with overlap leakage, and 32 with multi-test leakage.


\subsubsection*{Analyzing efficiency (RQ2).}
For efficiency, we recorded the execution time of our analysis for \emph{all} notebooks in our GitHub corpus. We record timing separately for the analysis front end (collecting facts), the type inference, and the actual analysis (datalog engine). We set a timeout of 5 minutes per notebook.
The experiment is conducted on a Precision 3650 workstation, with Intel(R) Xeon(R) W-1350 CPU and 32GB memory. The time is measured using Python's time module (wallclock time).

\subsubsection*{Analyzing leakage frequency (RQ3).}
We analyze leakage for the entire corpus and report the frequency with which we raise warnings for each kind of leakage. Note that we consider at most one warning per leakage kind per notebook to avoid biasing results with some notebooks that raise lots of warnings.

To further understand whether leakage associates with certain types of notebooks, we separately report leakage for different subpopulations. Specifically, we break down results for the following subpopulations:
\begin{itemize}
\item \emph{Popular notebooks} are viewed (and possibly reused) by more people, thus having more potential to spread problematic practices. We conjecture that popular notebooks come from more experienced data scientists and are better crafted. We identify 920 such popular notebooks as those in GitHub repositories in our corpus with 10 or more stars. 
\looseness=-1
\item \emph{Tutorial notebooks} similarly are explicitly designed for teaching others and could spread problematic practices. We identify \numprint{1157} tutorial notebooks by searching for the phrase \textit{``this tutorial''}. 
\looseness=-1
\item \emph{Assignment notebooks} contain solutions to course projects and assignments. We conjecture that these notebooks better represent practices of beginners than average notebooks in our corpus.
We identify \numprint{7576} assignment notebooks on GitHub by  searching for the keywords \textit{`homework'} and \textit{`assignment.'}
\item \emph{Competition notebooks (popular and recent)} are written by a mix of experienced and learning data scientists, possibly with an increased incentive to maximize model accuracy. Here, we report results from the Kaggle notebooks from our corpus.
\end{itemize}

\subsubsection*{Analyzing leakage characteristics (RQ4).}
% \todo{describe what exactly we measure and why, e..g, how do you measure lines of code and distance}
We measure distance between different program constructs by measuring lines of code between them (based on the Python files converted from notebooks using \textit{nbconvert} in the default setting) and compare them to the length of the entire notebook.
We expect that issues that span longer distances are harder to analyze manually.
Specifically, we calculate distance between leakage sources (e.g., reduced data) and training locations for preprocessing leakage, 
and distance between different evaluation locations for multi-test leakage.
We report the results for the entire GitHub corpus. 
% and again break it down by the same subpopulation as in RQ3.

For the whole dataset and each sub-population, we explore the distributions of different leakage issues, complexities of these issues, 
and also how they are distributed across different sub-populations.

\subsubsection*{Threats to validity.}
Establishing accurate ground truth for leakage is challenging. Our experience shows that even data science experts looking for leakage may miss it in complex data flows. We adopt a best effort approach with human labeling and comparisons with automated results that balance effort with confidence. We share our data for independent validation.

For RQ3 and RQ4, we report leakage warnings but validating all warnings is simply infeasible at this scale. Our results should therefore be interpreted with the error margins established in RQ1.
In addition, warnings about multi-test leakage may be rooted in settings where independent test data may exist outside of the notebook; our evaluation would also not detect multi-test leakage if the same test data was used repeatedly in past versions of a notebook or is used repeatedly in multiple notebooks. Generally, our analysis provides only a piece of a larger picture that needs to involve process design and other assurances, as we will discuss in Section~\ref{sec:discussion}.

The notebook population in our corpus is representative of public notebooks on GitHub (and some Kaggle competitions), but may not generalize to data science code outside of notebooks, across multiple notebooks, or to proprietary data science pipelines. Readers should hence be careful when generalizing our results.

Finally, our analysis focuses on the presence of leakage, not whether data scientists find leakage reports actionable or what effect leakage has in overestimating the reported accuracy results. 
We leave such evaluations to future work but point again to the fact that leakage is firmly established as problematic in educational material (cf. Sections~\ref{sec:intro}--\ref{sec:overfitting}).


% Note that the figures reported in Table~\ref{tab:leakage} may be higher than the actual figures,
% mainly because we assume that the notebooks are self-contained,
% i.e., all the training/validation/test data is directly used in the notebooks.
% In some settings (e.g., competitions), the labels of test data
% are often hidden from the participants.
% Other settings may restrict model developer access to the final test data.
% In these scenarios, the detected problem may no longer be an issue,
% once the model is tested with a new test set.

% In the case of unknown new test set, the detected test data within notebooks actually serves the purpose of validation data.
% However, it should still be noted that leakage between training data and validation data is still problematic,
% since it defeats the purpose of using validation data to provide a less biased evaluation score in the model development process.






% \subsection{Dataset Overview}
% \begin{table}[ht]
% \begin{tabular}{lllll}
% \toprule
% Dataset & \#notebooks & LoC & \#stars &   \\
% \midrule
% GitHub (all) & 107603 & 410 (387) & 1.1 &  \\
% GitHub (popular) & 920 & 378 (244)  & 95.2 &  \\
% GitHub (tutorial) & 1157 & 584 (332) & 4.2 &  \\
% GitHub (assignments)& 7576 & 559 (589) & 0.6  & \\
% % GitHub (competitions) &  &  &  &  \\
% Kaggle (top) & 312 & UNK854 & N/A &  \\
% Kaggle (recent) & 358 & UNK440 & N/A & \\
% \bottomrule
% \end{tabular}
% \caption{Dataset Overview. LoC is the average number of lines of code across all notebooks in the group.
% Number of stars is based on the repository that these notebooks reside in and is also averaged.}
% \label{tab:dataset}
% \end{table}


% From GitHub, we found 81379 repositories in September 2021 that contain notebooks.
% From these repositories, we found 107603 notebooks using targeted libraries (sklearn, keras, and pytorch).
% We further found three different sub-populations:
% notebooks from data science learners (assignments and homework),
% notebooks serving as tutorials,
% and notebooks from popular repositories .
% From Kaggle, we collected the top 200 and recent 200 notebooks from two competitions respectively.
% We also filtered them based on the libraries they use.
% In Table~\ref{tab:leakage}, we show basic statistics of all collected notebooks (repositories).


\subsection{Results}

\subsubsection{Analysis accuracy (RQ1)}
Our analysis prototype successfully executed for 94 of the 100 notebooks in our labeled RQ1 sample; the remaining 6 notebooks failed due to syntax errors. For the 94 notebooks, our prototype found 15 with preprocessing leakage, 7 with overlap leakage, and 19 with multi-test leakage.
All the found leakage issues were true positives except for one case due to over-approximation in related-data analysis, yielding a precision of 97.6\% (40 out of 41 detected issues).


\looseness=-1
On the other hand, our prototype missed 19 issues due to unsupported libraries~(6),
mistaking single test cases as test data (3), storing/loading model in external storage~(3), undetected test data evaluation (3), 
inaccurate type inference (2), and under/over-approximation in related-data analysis (2). This yields a recall of 67.8\% (40 out of 59).

\emph{Overall, our prototype achieves an accuracy of 92.9\% (262 out of 282 potential leakages).}
Analysis for preprocessing/overlap leakage is more accurate than multi-test leakage in this sample. 
Based on these results, we conclude that our analysis is generally accurate. 
% and could be further applied to a large set of notebooks.

% For these 55 notebooks, our analysis searched for three major types of leakage we discussed before. In xx of them, the analysis found at least one potential data leakage.

\subsubsection{Analysis overhead (RQ2)}

% \begin{table}[t]
% \begin{tabular}{lllll}
% \toprule
% component & avg. time (s)  & median time (s)  & fraction (\%) &  \\
% \midrule
% front-end & 0.03 & 0.02 & 0.81 &  \\
% type inference & 2.20 & 2.18 & 76.43 &  \\
% core analysis & 1.00 & 0.49 & 22.77 &  \\
% \bottomrule
% \end{tabular}
% \caption{Analysis overhead of Successfully Analyzed Notebooks.}
% \label{tab:time}
% % \vspace{-2.5em}
% \end{table}

% \begin{figure}[t]
%     \centering
%   \includegraphics[width=0.9\columnwidth]{images/time.pdf}
%   \vspace{-2.5em}
% \caption{Our analysis completes within 3.23 seconds on average, with most (76.43\,\%) of the time spent on type inference.}
% \label{fig:time}
% \vspace{-1em}
% \end{figure}


Most (92.78\,\%) of the 107,603 GitHub notebooks in our corpus could be analyzed successfully within the 5 minute time limit.
On average, our analysis completes within 3.23 seconds, with most of the time (2.20 seconds on average) spent on type inference.
% (Fig.~\ref{fig:time}). 
A small percentage of notebooks could not be analyzed due to
syntax errors (7.08\,\%), timeout (0.09\,\%; usually due to explosion from context-sensitivity in our data-flow analysis), and language features not supported by the front-end parser (0.05\,\%, e.g., named expression introduced in PEP 572).
\emph{We conclude that our analysis is efficient enough for interactive use and in continuous integration settings.}


% GitHub (all) & 107603 & 410 (387) & 1.1 &  \\
% GitHub (popular) & 920 & 378 (244)  & 95.2 &  \\
% GitHub (tutorial) & 1157 & 584 (332) & 4.2 &  \\
% GitHub (assignments)& 7576 & 559 (589) & 0.6  & \\
% % GitHub (competitions) &  &  &  &  \\
% Kaggle (top) & 312 & UNK854 & N/A &  \\
% Kaggle (recent) & 358 & UNK440 & N/A & \\

\subsubsection{Leakage in public notebooks (RQ3)}
\label{sec:empirical-study}

Our analysis reports at least one form of leakage for almost a third of all public notebooks in our GitHub corpus (29.6\%, see Table~\ref{tab:leakage}). \emph{We found frequent evidence of all three forms of leakage.}

\emph{Preprocessing leakage is prevalent in notebooks.}
Overall, our analysis reported preprocessing leakage for 12.3\% of notebooks in our corpus.
The most common sources of leakage during preprocessing are scaling, computing mean and standard deviation, and using results of a principal component analysis (PCA) in downstream data transformations.
For text data, the most common source of preprocessing leakage is vectorizing through counting or \emph{tf-idf} over the whole dataset. 
Zooming in, we reported preprocessing leakage in 32.9\% of those notebooks that scale their data, 8.4\% of those that compute mean or standard deviation, and 13.4\% of those that perform PCA.
% \cynote{among all leakage??}

\emph{Many notebooks lack independent test data.}
We report multi-test leakage in 18.5\% of all notebooks in our corpus. 
% We found that xx\% notebooks explicitly use APIs for hyper-parameter tuning.
We also detected that among all notebooks that train a model, 53.9\% contain validation data
(i.e., data that is used repeatedly for evaluation), but 35.0\% of trained models are not evaluated with \textit{independent} test data. 
Models evaluated with validation but without test data represent 28.3\% of all trained models in our GitHub corpus.

\emph{Training data often overlaps with validation and test data.}
We report overlap leakage in 6.5\% of all notebooks in our corpus. 
A closer look reveals that 8.0\% of all trained models are only evaluated on data that overlaps with its training data.


% [explain that multi-test leakage is sometimes not accurate when there is hidden test set]

\emph{Leakage is common in both beginner and expert code.}
When analyzing the subsets of our corpus, we report leakage in all subsets,
but to different degrees (see Table~\ref{tab:leakage}).
Assignment notebooks more representative of beginners are more likely to receive reports for all leakage types. In contrast, popular notebooks and tutorials
most likely associated with more advanced data scientists are slightly 
less likely to receive leakage reports, but leakage is still reported fairly commonly (20.9\,\% of popular and 16.2\,\% of tutorial notebooks). The fact that leakage seems common even in tutorial notebooks designed for educational purposes seems concerning.

Finally, the rate of reports of preprocessing leakage is very high in competition notebooks (>55\,\%). 
Indeed, it is not uncommon that competitors concatenate separately provided train and test data before preprocessing the combined dataset.
% as in Fig.~\ref{code:kaggle}. 
The way the competitions are designed (providing values but not labels of test data) may encourage exploiting leakage to maximize accuracy results, even, or especially by, experts. 
At the same time, because test labels are not provided, we do not report overlap and multi-test leakage. We will discuss competitions separately in Section~\ref{sec:discussion-kaggle}.


% \begin{figure}[t]
% \begin{lstlisting}[language=Python] 
% # Join train and test datasets
% dataset =  pd.concat(objs=[train, test], axis=0).reset_index(drop=True)

% # Fill Fare missing values with the median value
% dataset["Fare"] = dataset["Fare"].fillna(dataset["Fare"].median())
% \end{lstlisting}
% \caption{Leakage in Top competition solutions}
% \label{code:kaggle}
% % \vspace{-2em}
% \end{figure}


\subsubsection{Leakage characteristics (RQ4)}
We observe that leakage often occurs in patterns that make it challenging to detect manually.


\begin{figure}[t]
\begin{subfigure}[t]{0.45\columnwidth}
    \centering
  \includegraphics[width=\columnwidth]{images/frac.pdf}
  \caption{Distribution of fraction of distance between  preprocessing leak sources and training data.}
  \label{fig:frac1}
\end{subfigure}
\quad
\begin{subfigure}[t]{0.45\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{images/frac2.pdf}
  \caption{Distribution of fraction of distance between test locations that evaluate the same data.}
  \label{fig:frac2} 
\end{subfigure}
\caption{Leakage issues exhibit non-local pattern.}
\label{fig:frac}
\vspace{-2em}
\end{figure}


\emph{Leakage issues exhibit non-local patterns.}
For preprocessing leakage, the average distance between the leakage source (the \textit{reduce} edge) and the location where the training data is used is 293~lines of code.
In more than half of the cases, the distance between leakage source and training location is more than 20\% of the length of the notebook (see Fig.~\ref{fig:frac1}).
This distance illustrates the often long processing sequences and non-local data flows that are difficult to analyze manually.

% The average LoC between overlapping train/test data is 10.
% \cynote{track the distance between train/test and earliest dataset}

\looseness=-1
For multi-test leakage, the average distance between two locations evaluating models with the same (or related) data is 255~lines of code.
In more than 30\% of all cases, test location distance is more than 20\% of the whole notebook (see Fig.~\ref{fig:frac2}).
On average, there are 4.4 model-evaluation locations that use the same (or related) test data in notebooks with a multi-test leakage warning. This similarly illustrates the non-local reasoning required to notice this form of leakage.

% We do not track complexity of overlap leakage, as it is hard to trace back to the source where leakage is introduced.
% However, the flow-graph itself is already complex and hard to track


% For a small sample of notebooks, we also calculate the shortest data-flow path from leakage source to train/test locations,
% where the average path length is 4.
% More than x\% of them flow across method boundaries with an average of x times.
% These indicate that leakage issues are usually non-local, resulting from code in very different places,
% which makes it non-trivial for model developers to notice such issues.

\emph{A single notebook often trains multiple models.}
Among all notebooks in our GitHub corpus, 65.3\% train at least one model (in sklearn, pytorch, or keras) and 66.0\% evaluate at least one model (5.8\% of notebooks do not train but evaluate a model, typically when loading a pre-trained model).
Among the notebooks that do train at least one model, we found that 54.3\% train multiple models.
Having to commonly track multiple models and how data flows into their training and evaluation can be another challenge when manually reasoning about leakage.




% \subsection{Leakage in Competition Solutions (RQ3)}



% To understand leakage issues more accurately, we further perform a case study on competition solutions.
% In this setting, test data is explicitly given to the participants without labels.
% Therefore, it is inherently impossible to leak test data through either overlaps or multi-uses.
% However, since test data distribution is known, 
% there may still be preprocessing leakage in these solutions.

% In our result, we found that many competition solutions do leak test data in the preprocessing stage,
% and the fraction is much higher than average GitHub notebooks.
% Top voted notebooks and recent ones are similar in this regard (see Table~\ref{tab:leakage}).
% This indicates that competitors tend to use available test data information, even when they are experts.
% Indeed, it is not uncommon that competitors concatenate train and test data by themselves, and then preprocess the dataset (see Fig.~\ref{code:kaggle}).



% There are even several articles discussing how to exploit test data information in certain competitions,
% in order to get a higher test score~\cite{}.

% data: 100/179 recent ones & 87/156 top ones

% Similar to GitHub notebooks, Kaggle solutions exhibit similar leakage sub-patterns:



==> body/4-discussion.tex <==
%!TEX root = ../main.tex

\section{Discussion}
\label{sec:discussion}

Our results indicate that static detection of several forms of data leakage is feasible and that this kind of leakage is pervasive in practice. 
At the same time, it is not a comprehensive solution to avoid leakage or other forms of overfitting. 


% Therefore, when splitting ahead is infeasible for product team, or when model developers are collecting their own data, 
% it is advised that they should follow the best practice for model development.
% First, always split data first before any preprocessing, this prevents leaking through preprocessing.
% Second, use pipelines for preprocessing to avoid repetitive code. The pipeline should be fitted on training data and then used to transform test data.
% Finally, always make sure that there is an independent test set in the end, which should be evaluated only once.


% \subsection{Feedback from Instructors and Practitioners}
% We presented our prototype to instructors and industry practitioners. We ask for their feedback
% regarding to whether they will perceive it helpful.


% \cynote{
% Evaluate usefulness:
% \#1: show it to instructors [at CMU/over Internet] (simpler) 
% \#2: show it to industry practitioners (preferred)
% \#3: send pull requests/issues to popular demos 
% }



\subsection{Practical Impact of Data Leakage}
% As we have discussed before, not all leakage issues are equally problematic.
% Overlap leakage could cause serious overfitting, but the influence of multi-test leakage or preprocessing leakage might be less.
Not all leakage issues are equally problematic and some data scientists developing models may consider that some forms of leakage (e.g., the median of a column) are entirely negligible and that therefore warnings about leakage are not actionable and hence \emph{effective false positives}~\cite{tricorder}.
We even found some tutorials where the description explicitly indicates that developers are aware of leakage problems but ignore them anyway, such as 
testing with part of the training data ``for the sake of simplicity''.
% or explicitly merging validation and test data \todo{because... I did not get this?}.

% For example, we found some tutorials, where our analysis reports overlap leakage (i.e., they are testing on (part of) training data), explicitly claim that they do not perform data splits for the sake of simplicity.
% Other tutorials also explicitly mix validation data and test data.
% When validation data is not explicitly used for hyper-parameter tuning, this might not effectively cause leakage.


We have seen and heard of a large range of different impacts. On the one hand, we have heard (personal communication) of multiple cases where models were accidentally evaluated on training data producing entirely misleading results in research teams at BigTech companies, and that it is easy to create artificial examples where preprocessing leakage creates substantially inflated accuracy results (e.g., Fig.~\ref{fig:leak_acc}). On the other hand, experiments with notebooks in our corpus often just yielded marginal if any differences in accuracy.\footnote{Due to the known problems of reproducing public notebooks~\cite{pimentel2019large, wang2020assessing}, we were not able to perform systematic experiments on a larger sample.}

We expect that more substantial leakage, such as evaluating on the training data mostly stems from simple mistakes (such as using the wrong variable name) -- which \emph{practitioners} can easily detect with our analysis. The more subtle leakage through preprocessing may often have little effect on reported accuracy in most cases, but we still argue that it represents a bad coding pattern.
In our evaluation, we found that even many tutorials and top competition solutions leak their test data, let alone homework assignments.
We think that in particular \emph{educators} should insist on avoiding leakage in their course materials and homework, and our analysis provides an easy way to create awareness of the most common patterns leading to leakage.\footnote{We see some practitioners and educators agree with this stance. For example, in this GitHub issue (\url{https://github.com/keras-team/keras/issues/1753}), participants actively discuss the potential problems of
tutorials setting a bad example for learners, even when there technically is no actual leakage problem in the specific example. 
}

% Educators need to urge students to follow the best practices through setting good examples in their course materials.
% Library developers need to explicitly warn users against leakage patterns (as in the case of sklearn and imblearn),
% while avoiding being misleading in their own tutorials.

% \cynote{Does leakage matter: effect size (do experiments)?}






\subsection{Process Design for Preventing Data Leakage}
While we intend our analyzer to be used primarily as an educational tool and a tool to surface common mistakes in practice (either directly in notebook environments or integrated into code reviews~\cite{tricorder}), a more robust solution can be achieved by designing the process of how responsibilities are assigned. This is particularly relevant in formal settings where model development is outsourced~\cite{nadiaICSE22} and in data science competitions.

\subsubsection{Contract settings.}
In settings where a team is given data to develop a model as part of a contract (e.g., outsourcing), data leakage can systematically be avoided if test data is not provided to the data scientists who develop the model in the first place, but instead reserved for external evaluation upon delivery. 
When data scientists do not have access to test data, they cannot derive any insights from it, cannot use it repeatedly in evaluations, and cannot even manually look at data distributions to inform modeling decisions---even in settings where a data science team would have an incentive to cheat to present inflated accuracy numbers. 
The drawback of such a process design is that an additional external evaluator is needed who must have enough understanding of the data to be able to split it appropriately into training and test data (which can be nontrivial when dependencies exist~\cite{gorman-bedrick-2019-need, sogaard-etal-2021-need, splits-aiops,Saeb2017TheNT}). 
The evaluator also needs to have access to the model to run it locally, to not risk leaking test data during model inference. 
Also, the evaluator cannot repeatedly report results from the evaluation back to the developers of the model. Notice that test data does not become immediately useless, but gradually loses confidence which can be accounted for in scores, as explored in detail elsewhere \cite{renggli2019mlsys,thresholdout}.


\looseness=-1
In many practical settings though, the team developing the model is involved in acquiring or collecting the data in the first place~\cite{nadiaICSE22}. 
In such settings, it would be paramount for an external evaluator to independently collect data, which is often infeasible or prohibitively costly, as it might require replicating the expertise gained by the model development team during the development process. If there is some trust relationship between model developers and model users, approaches that foster best practices and avoid common mistakes, such as our static analysis tool, might be a better pragmatic alternative.

% Finally, the problem of leakage in \emph{offline} evaluations can be sidestepped entirely when testing \emph{online} with production data~\cite{worst-case-cite-my-blob-post,Kohavi2020TrustworthyOC,chaos-engineering} is feasible. Fresh production data could not have been used during model development and is hence unbiased. It also by definition comes from the target distribution 
% (avoiding certain pitfalls of shortcut learning~\cite{survey-on-shortcut-learning-from-seaibib}) 
% and is hence ideally suited to evaluate a model in the real production setting, rather than relying on offline evaluations. Unfortunately, evaluations in production are often difficult because ground truth labels are not available, expensive or can only be approximated, because of the risks of deploying poor-quality models in production, and because of the infrastructure overhead for testing in production.




% There are many ways to avoid data leakage, from better process designs to better code practice.
% Ideally, test data should be kept hidden from model developers. 
% In this way, we could guarantee that test data could not be exploited in the model development process.
% Indeed, a few Kaggle competitions keep test data hidden from competitors until the end of competition.
% During the competition, they show scores on a public test set (which is effectively validation data for model development) 
% in the leaderboard to help competitors improve their models.

\subsubsection{Data science competitions.}
\label{sec:discussion-kaggle}
Competitions often pursue a similar form of external evaluation, but often make compromises to better automate the competition, reduce cost and complexity, or increase engagement with more granular feedback:
% \begin{itemize}
% \item 

{\emph{Withholding test labels.}} A common design for Kaggle competitions is to provide test data without labels. The competitors submit the predicted labels to receive a test score. The operational advantage of this approach is that the competition organizer does not need to execute the submitted models---it avoids (1) executing submitted (untrusted) code, (2) having to support a range of different models, and (3) bearing the cost of model inference during evaluation. While this design prevents overlap leakage and multi-test leakage, preprocessing leakage is still possible. In fact, our evaluation of the two Kaggle competitions, which both use this design, shows that competitors often exploit preprocessing leakage.
% \item 

{\emph{Limiting repeated submissions.}} Most competitions allow participants to submit multiple revisions of a solution, receiving scores for each of them, risking multi-test leakage. To minimize this risk, some competitions limit the number of submissions per team. However, if participants can see other solutions in a leaderboard or create multiple accounts, leakage is still a concern even if the actual test data is withheld from competitors.
% \item 

\looseness=-1
{\emph{Partial test scores.}} Some competitions split their hidden test data and provide feedback on incremental submissions only with part of the test data, until finally scoring all submissions exactly once at the end of the competition with the remainder of yet unused test data. This effectively separates the hidden evaluation data into validation and test data. 
It still allows to provide meaningful preliminary feedback on a leaderboard during the competition, without allowing overfitting in the final results. As a downside, competitors that are better at extracting insights from partial test scores may have an advantage in the competition over those that just work with the training data, hence encouraging explicit attempts to leak information.
% \end{itemize}

While a once-only external evaluation with hidden test data at the end of the competition may be the cleanest solution, in practice competition designers will often want to make compromises with one of the designs above, which each reduce leakage to some extent but cannot avoid it entirely. Adding our static analyzer to the competition infrastructure could call out bad practices or could remind observers to not use the same practices outside competitions.

% Many competitions also only provide partial test score -- they show test score on part of test data in the public leaderboard, while the private leaderboard (i.e., test score on the rest of test data) is not visible until the end of competition.
% Note that this is different from the public/private test set design, as all test data (without labels) is still available but feedback is controlled.
% Beyond partial test score, approaches that systematically adjust test score to limit leakage's impact~\cite{renggli2019mlsys, thresholdout} could also be useful.
% Following such designs, we could avoid or mitigate \textit{Multi-test Leakage}, though competitors might still exploit distributional information from test data (i.e., \textit{Preprocessing Leakage}).

% Again, all these designs assume that training set and test set have already been separated, which requires nontrivial which might be easy for competition organizers.
% However, for product team, splitting data could be a tricky job.
% Random splits do not always work, as there may be dependencies between data points.
% In some settings, subject-wise splits might be more preferable~\cite{Saeb2017TheNT},
% while in other settings, splits along time axis would provide a more accurate evaluation.
% Even within research communities, how to split data is debated extensively~\cite{gorman-bedrick-2019-need, sogaard-etal-2021-need, splits-aiops}.



\subsection{API Design for Preventing Data Leakage}
It is also possible to avoid certain leakage issues through API design. For example, many ML libraries advocate the use of pipelines for preprocessing~\cite{scikit}. If correctly used, they could help avoid preprocessing leakage, because the library enforces that only training data is used to extract parameters for preprocessing.

From our GitHub corpus, we observe that only 5.5\% notebooks use pipelines. 
Surprisingly, 18.1\% of these notebooks still contain pre-processing leakage. 
When we inspected samples from these notebooks, we found that they often do not apply pipelines to the whole preprocessing stage, and some of them even use pipelines in the wrong way.
This informs us that better education on how to use these APIs is as important as designing these leakage-proof APIs themselves.


\subsection{Limitations and Alternatives}
Our definitions of leakage and corresponding analyses are limited to the scope of what is observable statically in data science code (typically in a notebook). In addition, our static approximation relies on models of library functions and several heuristics.

\looseness=-1
Importantly, our approach cannot detect repeated evaluations that are not present in the notebook (e.g., cells modified and evaluated repeatedly) and cannot detect test data outside the notebook. It may therefore issue spurious  multi-test leakage warnings or miss some. 
Our evaluation also shows that our analysis misses some leakage but produces few false positives (recall: 67.8\%, precision 97.6\%), therefore the reported leakage may be underestimated.
Similar to many static analysis warnings, we envision warnings as a starting point for reflection and discussion (e.g., during code review~\cite{tricorder}), and not necessarily as a blocking issue that always needs to be addressed with code changes.
For example, developers might compare several techniques on the same dataset, while the final test score is computed outside the notebook. Our approach would report such patterns, but these false positives should not affect the developer's workflow.

In an adversarial setting, it is easy to trick our analysis by for example using meta-programming or coding patterns that exceed the capabilities of our analysis (e.g., store and load data in a file). 
Additional rules and environment models can strengthen our analysis but will not overcome fundamental limitations. 
A sound analysis for an adversarial setting may be possible but would likely be so restrictive or create so many false positives to render the approach impractical.
Again, our analysis is not a safeguard against all kinds of cheating in data science competitions. It better serves as a lightweight checker that discourages bad practices of data leakage.

Dynamic analysis could improve accuracy in many cases, for example tracking the origin of individual rows in the data rather than our approximations in the related-data relationship. However, dynamic analysis would require the entire notebook to be executed for analysis (with the induced overhead), which can be costly in many machine learning tasks and may not be feasible when studying public notebooks that are often hard to reproduce~\cite{pimentel2019large}.



==> body/5-related-works.tex <==
\section{Related Work}


\paragraph{Quality Assurance for Data Science Code}
Prior work has noted that data science code is often of low quality---%
relying heavily on copied code and code clones~\cite{koenzen2020code},
ignoring basic coding and style conventions~\cite{zeller-icse20-nier},
being poorly documented~\cite{painpointspaper}, 
containing frequent bugs in data transformations~\cite{chenyangASE21},
and being hard to reproduce~\cite{pimentel2019large,wang2020assessing}.
In a well-known article, \citet{Sculley2015HiddenTD} have argued that data science code is particularly prone to accumulating technical debt due to complexity and often poor engineering practices.
Our work on data leakage explores another common quality issue that may lead to unreliable accuracy evaluations.
% Similar to other tools that help data scientist write better code~\cite{wang2021restoring, head2019managing,chenyangase}, 
% our analysis tooling is intended to improve practices and code quality in data  science projects. 

% \cynote{not sure whether needed: cite many se4ds papers: technical debts, }
% \todo{I'd cite at least the technical debt paper and a few that complain about the code quality of data science code -- we help here }

\paragraph{Static Analysis for Python}
% \citet{li2022scalpel}
Despite its popularity, there are relatively few static analysis frameworks or tools written for Python,
partly due to the difficulties of handling Python's dynamic features.
%  proposes a static analysis tool in TypeScript that could extract def-use graph from given Python code.
\citet{head2019managing} implemented a static def-use analysis for Python to perform program slicing that helps data scientists clean, recover, and compare versions of code.
\textit{Scapel}~\cite{li2022scalpel} is a static analysis framework written in Python that integrates several common analyses (e.g., alias analysis).
\textit{NBLyzer}~\cite{DBLP:journals/corr/abs-2110-08339} is a framework specifically written for notebook code in Python, 
where they focus on supporting notebook actions (e.g., code changes, cell executions).
Pysa~\cite{pyre} is a taint analysis tool that aims to identify potential security issues in Python code.
~\citet{tensorflowshape20} proposed a static shape analysis for Tensorflow programs, which is integrated into the \textit{doop} framework.
We chose to develop our own analysis, because it gives us the flexibility to tailor it for the purpose of leakage detection,
where we need to track several custom relations.
% Our prototype was also developed in the same time of the two proposed frameworks.

% \cynote{type inference??}

\paragraph{Data Leakage Detection}
\looseness=-1
Data leakage detection is a largely unexplored problem.
\citet{kaufman2012leakage} discuss how to manually perform analyses to detect certain kinds of data leakage in raw data, in particular label leakage.
% (where an input feature correlates with the label; a form of shortcut learning). 
\textit{Deepchecks}~\cite{deepchecks} is a library that aims to validate machine-learned models and data, which
supports dynamic check for overlap leakage between train and validation/test set by dynamically inspecting datasets (e.g., whether test data contains rows that occur identically in training data). 
Closest to our work is a customized analysis to detect preprocessing leakage in the \textit{NBLyzer}~\cite{DBLP:journals/corr/abs-2110-08339} framework.
However, their data leakage analysis is just a demonstration for their framework and does not capture the full complexity of data leakage.
For example, they do not establish data-model mappings but assume that all training/test locations are relevant globally (i.e., connected by the same/related models).
They also do not actively distinguish validation data from test data, or track whether variables might be aliased.
This results in a leakage specification that only poorly approximates the ground truth.
Because their implementation is not publicly available, we did not compare our approach with theirs in our evaluation.
% They assert that training data and test data should not have the same source variable 
% (which is the last source variable used in a in their flow path).
In contrast to prior work, we detect multiple forms of data leakage and also detect leakage accurately even when datasets are transformed.

% Similar to Deepchecks, there are also many works that detect data smell ~\cite{data-linter}.


\paragraph{Provenance Tracking for Data Science Code}
Provenance tracking in data science code has been studied extensively~\cite{Vamsa, pimentel2017noworkflow}.
Most relevant are approaches that track origins of data at the row level in data analytics code for various frameworks: Titian~\cite{titian} for Spark, RAMP~\cite{ramp} for Hadoop, and Newt~\cite{newt} for Hadoop and Hyracks.
As discussed, we only statically approximate what could be tracked more accurately with dynamic record-level provenance tracking approaches, but these approaches need to instrument the frameworks to track provenance at runtime.
Overall, this kind of tracking is only a building block in our leakage detection.

% Goods paper; generalization of our prototype

% \cynote{not sure whether needed: Identifying map functions in arbitrary code in loop parallelization.}


\section{Conclusion}

% \cynote{longer conclusion?}

\looseness=-1
We provide a summary of common data leakage problems and propose a static analysis approach that could automatically detect them.
We find that leakage issues are common in public notebooks and provide recommendations on process designs to prevent data leakage.

==> body/approach-example.tex <==



\begin{figure*}[ht]
\begin{subfigure}[b]{\columnwidth}
\begin{lstlisting}[name=example]
import pandas as pd
from sklearn.feature_selection import SelectPercentile, chi2
from sklearn.model_selection import LinearRegression, Ridge
X_0, y = load_data()

select = SelectPercentile(chi2, percentile=50)
%\mytikzmark{leakStart}%select.fit(X_0)%\mytikzmark{leakEnd}%
X = select.transform(X_0)

X_train, y_train, X_test, y_test = train_test_split(X, y)
lr = LinearRegression()
%\mytikzmark{train1Start}%lr.fit(X_train, y_train)%\mytikzmark{train1End}%
lr_score = %\mytikzmark{test1Start}%lr.score(X_test, y_test)%\mytikzmark{test1End}%

ridge = Ridge()
%\mytikzmark{train2Start}%ridge.fit(X, y)%\mytikzmark{train2End}%
ridge_score = %\mytikzmark{test2Start}%ridge.score(X_test, y_test)%\mytikzmark{test2End}%

final_model = lr if lr_score > ridge_score else ridge
\end{lstlisting}
  \vspace{-1em}
\caption{\small This code contains all three types of data leakage.
Leakage-prone operations (reduce edges) and train/test locations are highlighted in red/yellow.
In lines 7-8, there is a preprocessing leakage, where it selects features based on both training data and test data.
In lines 16-17, there is an overlap leakage, where test data is used for training.
There is also a multi-test leakage because \textit{X\_test} is evaluated multiple times and there is no other independent test data.
}
\label{code:dataflow1}
\begin{tikzpicture}[remember picture, overlay]
        \highlight{train1Start}{train1End}
        \highlight{train2Start}{train2End}
        \highlight{test1Start}{test1End}
        \highlight{test2Start}{test2End}
        \highlightred{leakStart}{leakEnd}
\end{tikzpicture}   
\end{subfigure}
\hfill
\begin{subfigure}[b]{\columnwidth}
\begin{lstlisting}[name=example]
import pandas as pd
from sklearn.feature_selection import SelectPercentile, chi2
from sklearn.model_selection import LinearRegression, Ridge
X_0, y = load_data()

X_train_0, y_train, X_test_0, y_test = train_test_split(X_0, y)
select = SelectPercentile(chi2, percentile=50)
%\mytikzmark{leak2Start}%select.fit(X_train_0)%\mytikzmark{leak2End}%
X_train = select.transform(X_train_0)
X_test = select.transform(X_test_0)

lr = LinearRegression()
%\mytikzmark{train3Start}%lr.fit(X_train, y_train)%\mytikzmark{train3End}%
lr_score = %\mytikzmark{test3Start}%lr.score(X_test, y_test)%\mytikzmark{test3End}%

ridge = Ridge()
%\mytikzmark{train4Start}%ridge.fit(X_train, y_train)%\mytikzmark{train4End}%
ridge_score = %\mytikzmark{test4Start}%ridge.score(X_test, y_test)%\mytikzmark{test4End}%

final_model = lr if lr_score > ridge_score else ridge
X_test_new_0, y_test_new = load_test_data()
X_test_new = select.transform(X_test_new_0)
%\mytikzmark{test5Start}%final_model.score(X_test_new, y_test_new)%\mytikzmark{test5End}%

\end{lstlisting}
  \vspace{-1em}
\caption{\small We could fix the code on the left by
moving feature selection later (after train/test splits),
using only training data for training \textit{ridge},
and using independent test data for evaluation in the end.
}
\label{code:dataflow2}
\begin{tikzpicture}[remember picture, overlay]
        \highlight{train3Start}{train3End}
        \highlight{train4Start}{train4End}
        \highlight{test3Start}{test3End}
        \highlight{test4Start}{test4End}
        \highlight{test5Start}{test5End}
        \highlightred{leak2Start}{leak2End}
\end{tikzpicture}  
\end{subfigure}

\begin{subfigure}[b]{\columnwidth}
   \centering
  \includegraphics[width=0.75\columnwidth]{images/dataflow_a.pdf}
  \vspace{-1em}
  \caption{\small Data-flow graph for the code. Only important variables are shown. 
  Edges between datasets are solid, while other edges are dotted. 
  Reduce edges, together with their variables, are marked in red. 
}
  \label{fig:dataflow}
\end{subfigure}
\hfill
\begin{subfigure}[b]{\columnwidth}
   \centering
  \includegraphics[width=\columnwidth]{images/dataflow_b.pdf}
  \caption{\small Data-flow graph for the code after fix. 
  \textit{X\_train\_0} is no longer related to \textit{X\_test}, eliminating the preprocessing leakage.
  With changes to training data and the introduction of a new test dataset,
  the overlap leakage and multi-test leakage are also fixed.
}
  \label{fig:dataflow2}
\end{subfigure}
\caption{Example code with data-flow graph (before and after fix) for leakage analysis.}
\label{fig:approach_example}
% \vspace{-1em}
\end{figure*}


==> body/datalog.tex <==

\begin{figure}[t]
\small

\begin{tabular}{l}

\textbf{Inputs} \hfill \\
 $\mathbf{V}$ \hfill program variables  \\
 $\mathbf{D} \subseteq \mathbf{V}$ \hfill datasets  \\
 $\mathbf{M} \subseteq \mathbf{V}$ \hfill models  \\
 $\textit{DataFlow} \subseteq \*V\times \*V$ \hfill data flow paths (transitive closure)  \\
%  & transitive closure of flow edges\\
%  , $\textit{MapPath} \subset \textit{DataFlow}$
 $\textit{DatasetFlow} \subseteq \*D\times \*D$ \hfill data flow paths between datasets \\
 $\textit{MapEdge} \subseteq \*D\times \*D$ \hfill map-like operations \\
 $\textit{ReduceEdge} \subseteq \*D\times \*V$ \hfill reduce-like operations \\
 $\textit{DupEdge} \subseteq \*D\times \*D$ \hfill duplication operations \\
 $\textit{ModelData} \subseteq \*M\times \*D\times \mathcal{P}(\*D)\times  \mathcal{P}(\*D)\quad$ \hfill models with corresponding \\
 \hfill training, validation, and test datasets \\
 \\
 
\textbf{Rules} \hfill \\
%  $\textit{RelData} \subseteq \*D\times \*D$ \hfill related-data relation \\


 %   $\textit{LeakedModel} \in \*M$ & models with leakage \\
%   $\textit{model}: \*T \rightarrow \*M$ & get model \\
%  $\textit{train}: \*T \rightarrow \*D$ & get training data \\
%  $\textit{val}: \*T \rightarrow [\*D]$ & get a list of validation data \\
%  $\textit{test}: \*T \rightarrow [\*D]$ & get a list of test data \\
 
\end{tabular}

\footnotesize
\[
    \begin{array}{c}  \\
      \inference{a \in \*D \quad b\in \*D\quad (a, b) \in \textit{DatasetFlow}}
      {(a, b) \in \textit{RelData}}[reldata/flow]
      \\[1.5em]
      \inference{(b, a) \in \textit{RelData}}
      {(a, b) \in \textit{RelData}}[reldata/sym] 
      \hspace{2em}\inference{a \in \*D}
      {(a, a) \in \textit{RelData}}[reldata/ref] 
      \\[1.5em]
      \inference{(a, b) \in \textit{RelData}\quad (a, c) \in \textit{RelData}\quad (a, c) \in \textit{MapEdge}}
      {(b, c) \in \textit{RelData}}[reldata/map]
      \\[1.5em]
      \inference{(src, a) \in \textit{DupEdge}\quad (a, b) \in \textit{RelData}\quad (a, c) \in \textit{RelData}}
      {(b, c) \in \textit{RelData}}[reldata/dup]
      \\[1.5em]
      \inference{\exists(m, d_\textit{tr}, D_\textit{va}, D_\textit{te})\in \textit{ModelData},\; D_\textit{va} \neq \varnothing\\ \forall (m, d_\textit{tr}, D_\textit{va}, D_\textit{te})\in \textit{ModelData},\; D_\textit{te} = \varnothing}
      {\textit{multi-test leakage in notebook}}[leak/multi] 
      \\[1.5em]
      \inference{(m, d_\textit{tr}, D_\textit{va}, D_\textit{te})\in \textit{ModelData}\\ \forall d_e\in D_\textit{te}\cup D_\textit{va}, (d_e, d_\textit{tr})\in \textit{RelData}}
      {\textit{leakage due to overlap between $d_\textit{tr}$ and $D_\textit{te}\cup D_\textit{va}$ for model $m$}}[leak/overlap]
      \\[1.5em]
      \inference{(m, d_\textit{tr}, D_\textit{va}, D_\textit{te})\in \textit{ModelData}\quad
      (s, t) \in \textit{ReduceEdge} \\ d_\textit{e}\in  D_\textit{te}\cup D_\textit{va}\quad (d_\textit{e}, s) \in \textit{RelData}\quad (t, d_\textit{tr})\in \textit{DataFlow} }
      {\textit{leakage between $d_\textit{tr}$ and $d_\textit{e}$ through the transformation from $s$ to $t$}}[leak/pre] 
    \end{array}
  \]
  \vspace{-1em}
  \caption{Notations and rules for leakage detection from input relations.}
  \label{fig:rules}
%   \vspace{-1em}
\end{figure}

% \begin{figure*}[ht]
% \begin{subfigure}[b]{\columnwidth}



% % \begin{lstlisting}[language=C, numbers=none]

% \textsc{Domains}
% \begin{tabular}{l}
%  $\mathbf{V}$ is a set of program variables  \\
%  $\mathbf{D}$ is a set of datasets, $\mathbf{D} \subset \mathbf{V}$  \\
%  $\mathbf{M}$ is a set of models, $\mathbf{M} \subset \mathbf{V}$ \\
%  $[\*X]$ is a set of lists, each list contains zero or more \\
%  elements from domain $\*X$
% \end{tabular}

% \textsc{Relations}
% \begin{tabular}{l}
%  \textit{RelatedData}$(a:\*D, b:\*D)$  \\
%  \textit{ModelData}$(model:\*M, trs:[\*D], vals:[\*D], tests:[\*D])$  \\
%  \textit{ReduceEdge}$(from:\*D, to:\*V)$ \\
%  \textit{FlowEdge}$(from:\*V, to:\*V)$ \\
%  \textit{Leakage}$(model:\*M, msg:\*V)$
% \end{tabular}

% \textsc{Rules}
% \begin{tabular}{l}
%  \textit{RelatedData}$(a, b)$ $\leftarrow$  \\
%  $\quad$ \textit{FlowEdge}$(a, b)$. \\
%  \textit{ModelData}$(model:\*M, train:\*D, val:\*D, test:\*D)$   \\
%  \textit{ReduceEdge}$(from:\*D, to:\*V)$ 
% \end{tabular}


% \begin{lstlisting}[language=C, numbers=none]
% // Relations
% .decl RelatedData(a:D, b:D)

% .decl TrainingData(model: Var, train: Var)
% .decl TestData(model: Var, test: Var)
% .decl TestScoreData(model: Var, test: Var)
% .decl ValData(model: Var, val: Var)

% // aggregation
% .decl ReduceEdge(to: Var, from: Var)

% // Analysis results
% .decl VarPointsTo(var: Var, heap: Value)
% .decl FlowFrom(to:Var, from:Var, tag:symbol)
% // Output
% .decl PreProcessingLeak(model:Var, train: Var, test: Var)
% .decl OverlapLeak(model:Var, train: Var, test: Var)
% .decl NoTestData(model:Var, train: Var)
% \end{lstlisting}

% \begin{lstlisting}[language=C]
% // Overlap detection
% DataOverlap(train, test) :-
%     FlowFrom(train, test, _);
%     FlowFrom(test, train, _).

% DataOverlap(train, test) :-
%     DuplicateEdge(des, src),
%     FlowFrom(train, des, _),
%     FlowFrom(test, des, _).

% DataOverlap(train, test) :-
%     DuplicateEdge(des, src),
%     FlowFrom(train, des, _),
%     (FlowFrom(test, src, _);
%     FlowFrom(test, src_equiv, _), 
%     FlowFrom(src, src_equiv, "equiv")).

% DataOverlap(train, test) :-
%     DuplicateEdge(des, src),
%     FlowFrom(test, des, _),
%     (FlowFrom(train, src, _);
%     FlowFrom(train, src_equiv, _), 
%     FlowFrom(src, src_equiv, "equiv")).
% \end{lstlisting}

% \label{code:dataflow}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{\columnwidth}
% \begin{lstlisting}[language=C]
% // Pairing training/test data
% TrainTestPair(trainModel, train, testModel, test) :-
%     TestData(testModel, test),
%     TrainingData(trainModel, train),
%     !DataOverlap(test, train),
%     FlowFrom(testModel, trainModel, _).
    
% // Pre-processing leak detection
% PreProcessingLeak(testModel, train, test) :-
%     TestDataWithModel(testModel, test),
%     TrainingDataWithModel(trainModel, train),
%     !DataOverlap(test, train),
%     FlowFrom(testModel, trainModel),
%     ReduceEdge(des, src),
%     FlowFrom(train, des, _),
%     DataOverlap(test, src).
    

% OverlapLeak(testModel, train, test) :-
%     TestDataWithModel(testModel, test),
%     TrainingDataWithModel(trainModel, train),
%     DataOverlap(test, train),
%     train != test, // ad-hoc ??
%     FlowFrom(testModel, trainModel, _).

% // Other Problems
% NoTestData(trainModel, train) :-
%     TrainingData(trainModel, train),
%     !TrainTestPair(trainModel, train, _, _).

% MultipleTestScoreLeak(train, test) :-
%     TestScoreData(testModel, test),
%     TestScoreData(testModel2, test2),
%     DataOverlap(test, test2),
%     FlowFrom(testModel2, testModel, _).
    

% \end{lstlisting}

% \end{subfigure}

%     \caption{Analysis rules}
%     \label{fig:analysis}
% \end{figure*}


==> body/intro-example.tex <==

\begin{figure}
% \centering \textit{Test data used for training}

% \begin{lstlisting}[language=Python]
% # test data used for tuning
% gs = GridSearchCV(lr, {'penalty': penalties, 'C': C_vals}, verbose=False, cv=15)
% gs.fit(X, y)
% logreg = LogisticRegression(C=gs.best_params_['C'], penalty=gs.best_params_['penalty'])

% X_train, y_train, X_test, y_test = train_test_split(X, y)
% cv_model = logreg.fit(X_train, Y_train)
% cv_pred = cv_model.predict(X_test)
% \end{lstlisting}
\begin{subfigure}[b]{\columnwidth}
\begin{lstlisting}[language=Python]
# oversampling datasets, new rows are synthesized based on existing rows
X_new,y_new = SMOTE().fit_resample(X,y)
# splits after over-sampling no longer produce independent train/test data
X_train, X_test, y_train, y_test = train_test_split(X_new, y_new, test_size=0.2, random_state=42)

rf = RandomForestClassifier().fit(X_train,y_train)
rf.predict(X_test)
\end{lstlisting}
\vspace{-1em}
\caption{\small Test data used for training}
\vspace{0.5em}
\label{code:overlap_example}
\end{subfigure}

% \begin{lstlisting}[language=Python] 
% # training data includes test data
% model.fit(X, y)
% X_train, y_train, X_test, y_test = train_test_split(X, y)
% model.score(X_test, y_test)
% \end{lstlisting}
% \begin{lstlisting}[language=Python]
% # tune hyperparameters with test data
% X_train, y_train, X_test, y_test = train_test_split(X, y)
% opt = GridSearch(model, param_grid)
% opt.fit(X_train, y_train, X_test, y_test)
% opt.score(X_test, y_test)
% \end{lstlisting}
% \begin{lstlisting}[language=Python]
% # augmentation before splits makes train/test data dependent
% X, y = oversampler.fit_sample(X_0, y_0)
% X_train, y_train, X_test, y_test = train_test_split(X, y)
% model.fit(X_train, y_train)
% model.score(X_test, y_test)
% \end{lstlisting}

% \centering \textit{Test data used repeatedly for model selection}
\begin{subfigure}[b]{\columnwidth}
\begin{lstlisting}[language=Python]
# select the best model with repeated evaluation
results = []
for clf, name in (
        (DecisionTreeClassifier(), "Decision Tree"),
        (Perceptron(), "Perceptron")):
    clf.fit(X_train, y_train) 
    pred = clf.predict(X_test) 
    score = metrics.accuracy_score(y_test, pred)
    results.append(score, name)
\end{lstlisting}
\vspace{-1em}
\caption{\small Test data used repeatedly for model selection}
\vspace{0.5em}
\label{code:multi_test_example}
\end{subfigure}

% \begin{lstlisting}[language=Python]
% # select the best model with repeated evaluation
% X_train, y_train, X_test, y_test = train_test_split(X, y)
% max_score = init()
% final_model = None
% for model in models:
%     model.fit(X_train, y_train)
%     s = model.score(X_test, y_test)
%     if s > max_score:
%         max_score = s
%         final_model = model
% \end{lstlisting}

% \centering \textit{Test data leaked in preprocessing}
\begin{subfigure}[b]{\columnwidth}
\begin{lstlisting}[language=Python]
# unknown words in test data leak into training data
wordsVectorizer = CountVectorizer().fit(text)
wordsVector = wordsVectorizer.transform(text)
invTransformer = TfidfTransformer().fit(wordsVector)
invFreqOfWords = invTransformer.transform(wordsVector)
X = pd.DataFrame(invFreqOfWords.toarray())

train, test, spamLabelTrain, spamLabelTest = train_test_split(X, y, test_size = 0.5)    
predictAndReport(train = train, test = test)
\end{lstlisting}
\vspace{-1em}
\caption{Test data leaked in preprocessing}
\label{code:pre_processing_example}
\end{subfigure}
% \begin{lstlisting}[language=Python]
% # test data distribution information leaks to training data
% X1 = normalize(X)
% X_train, y_train, X_test, y_test = train_test_split(X1, y)
% model = LinearRegression()
% model.fit(X_train, y_train)
% model.score(X_test, y_test)
% \end{lstlisting}

% \centering \textit{Data split in the wrong way}
% \begin{lstlisting}[language=Python]
% # random split of time-series data makes train/test data dependent
% X_train, y_train, X_test, y_test = train_test_split(X_time_series, y) # random split
% model.fit(X_train, y_train)
% model.score(X_test, y_test)
% \end{lstlisting}
\caption{Shortened data leakage examples from public notebooks.}
\label{fig:example}
\vspace{-2em}
\end{figure}



==> macros.tex <==
\usepackage{listings}
\lstset{
%        xleftmargin=0.5cm,
        extendedchars=true,
        basicstyle=\footnotesize\ttfamily,
        showstringspaces=false,
        showspaces=false,
        numbers=left,
        numberstyle=\footnotesize\ttfamily,
        numbersep=7pt,
        xleftmargin=2em,
        framexleftmargin=2em,
        tabsize=2,
        breaklines=true,
        showtabs=false,
        captionpos=b,
        language=python, 
        frame=lines, 
        commentstyle=\color{mygreen},
        escapeinside={\%}{\%},          % if you want to add LaTeX within your code
        keywordstyle=\color{blue},       % keyword style
        stringstyle=\color{mymauve},     % string literal style
        literate={\$}{{\textcolor{mymauve}{\$}}}1
}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{tikz}
\usetikzlibrary{tikzmark}
\usepackage{color}
\usepackage{enumitem}

\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

% Command to place a TikZ anchor at the current position
\newcommand{\mytikzmark}[1]{%
  \tikz[overlay,remember picture,baseline] \coordinate (#1) at (0,0) {};}

\newcommand{\highlight}[2]{%
  \draw[yellow,line width=8pt,opacity=0.3]%
    ([yshift=2pt]#1) -- ([yshift=2pt]#2);%
}
\newcommand{\highlightred}[2]{%
  \draw[red,line width=8pt,opacity=0.3]%
    ([yshift=2pt]#1) -- ([yshift=2pt]#2);%
}


\usepackage{diagbox}
\usepackage{tabularx}
\usepackage{booktabs}
\usepackage{semantic}
\usepackage{proof}
% \usepackage{paralist}
\usepackage{numprint}
\npdecimalsign{\ensuremath{\cdot}}
\npthousandsep{,}
% \nprounddigits{3}

\usepackage{soul}

\newcommand{\cynote}[1]{{\color{magenta} \small(\underline{Chenyang}: #1)}}
\newcommand{\cknote}[1]{{\color{violet} \small(\underline{Christian}: #1)}}
\newcommand{\glnote}[1]{{\color{blue} \small(\underline{Grace}: #1)}}
\newcommand\todo[1]{\textcolor{red}{#1}}
\def\*#1{\mathbf{#1}}


% \settopmatter{printacmref=false}
